ConEx: Efficient Exploration of Big-Data System Configurations for Better Performance

Configuration space complexity makes the big-data software systems hard to configure well. Consider Hadoop, with over nine hundred parameters, developers often just use the default configurations provided with Hadoop distributions. The opportunity costs in lost performance are significant. Popular learning-based approaches to auto-tune software does not scale well for big-data systems because of the high cost of collecting training data. We present a new method based on a combination of Evolutionary Markov Chain Monte Carlo (EMCMC) sampling and cost reduction techniques to cost-effectively find better-performing configurations for big data systems. For cost reduction, we developed and experimentally tested and validated two approaches: using scaled-up big data jobs as proxies for the objective function for larger jobs and using a dynamic job similarity measure to infer that results obtained for one kind of big data problem will work well for similar problems. Our experimental results suggest that our approach promises to significantly improve the performance of big data systems and that it outperforms competing approaches based on random sampling, basic genetic algorithms (GA), and predictive model learning. Our experimental results support the conclusion that our approach has strongly demonstrated potential to significantly and cost-effectively improve the performance of big data systems.

==> algo_accept.tex <==
\begin{algorithm}[t!]
    \removelatexerror
\small
  \caption{{Acceptance sub-routine of EMCMC}}
  \label{alg:emcmc-accept}

  \SetKwInOut{Input}{Input} 
   \SetKwInOut{Output}{Output}
   \SetKwRepeat{Do}{do}{while}
   
 \underline{Function Accept}   \\
  \Input{$perf_{best}, perf_{p}$} 
  \Output{bool: accept/reject $conf_p$}
     
    $\Delta perf$ $\leftarrow$ $\frac{perf_{best} - perf_{p}}{perf_{best}}$ \label{alg:emcmc-accept:compute_imp} \\
    $accept\_prob$ $\leftarrow$ $exp(\Delta perf)$ \label{alg:emcmc-accept:compute_acc_prob}\\
    \If{$Rand(0, 1) < accept\_prob$} {  \label{alg:emcmc-accept:compare_with_rand}
	    \Return{True}
    }
    \Return{False}
\end{algorithm}

==> algo_emcmc.tex <==

%\setlength\floatsep{1.25\baselineskip plus 3pt minus 2pt}


\begin{algorithm}[t!]
    \removelatexerror
\small
\setlength\textfloatsep{1\baselineskip plus 0pt minus 0 pt}
\setlength\intextsep{1\baselineskip plus 0pt minus 0 pt}
% \scriptsize
  \caption{{Explore Configuration Space with EMCMC}}
  \label{alg:mcmc-ga}

  \SetKwInOut{Input}{Input} 
   \SetKwInOut{Output}{Output}
   \SetKwRepeat{Do}{do}{while}
   
 \underline{Function EMCMC()}   \\
  \Input{Refined Configuration Space $\zeta$, \\
            job, \\
            seed configuration $conf_{seed}$, \\
            threshold max\_gen %, min\_improvement
            }   \label{alg:mcmc-ga:line:input}
  \Output{Best configuration $conf_{best}$, \\
          Corresponding performance $perf_{best}$}  \label{alg:mcmc-ga:line:ouput}

     $perf_{seed}$ $\leftarrow$ run $job$ with $conf_{seed}$ \label{alg:mcmc-ga:line:init_perf}\\
     $conf_{best}$ $\leftarrow$ $conf_{seed}$ \label{alg:mcmc-ga:line:init_best_conf} \\
     $perf_{best}$ $\leftarrow$ $perf_{seed}$  \label{alg:mcmc-ga:line:init_best_perf}\\
     $generation$ $\leftarrow$ $1$ \label{alg:mcmc-ga:init_gens}\\
     $\Delta perf$ $\leftarrow$ $0$ \label{alg:mcmc-ga:init_global_imp}\\
          $conf_{parents}$ $\leftarrow$  sample $n$ random configurations from $\zeta$ \label{alg:mcmc-ga:line:sample_fst_generation} \\
     \Do{generation $<$ max\_gen } { % ||$ $\Delta perf$ $>$ $min\_improvement$} {  
        $confs_{accepted}$ $\leftarrow$ $EmptyList$ \\
        \ForEach{parent $conf_p \in conf_{parents}$} { \label{alg:mcmc-ga:line:loop_start}
        		$perf_{p}$ $\leftarrow$ run $job$ with $conf_p$ configuration \label{alg:mcmc-ga:line:evaluate_confp} \\
        		$accepted$ $\leftarrow$ Accept($perf_{best}, perf_{p}$) \# based on Eq.~\ref{eq:m} \label{alg:mcmc-ga:line:accept} \\
        		\If{accepted} {
        		    $confs_{accepted}.add(conf_p)$ \label{alg:mcmc-ga:line:add_accepted} \\
                \If{$perf_p > perf_{best}$} { \label{alg:mcmc-ga:line:update_best_start}
                    $conf_{best} \leftarrow conf_p$ \\
                $perf_{best} \leftarrow perf_p$  
                } \label{alg:mcmc-ga:line:update_best_end}
        		} 
        }   \label{alg:mcmc-ga:line:loop_end}
        $\Delta perf$ $\leftarrow$ $(perf_{best} - perf_{seed})/perf_{seed}$ \label{alg:mcmc-ga:update_global_imp}\\
        $conf_{parents} \leftarrow evolve(conf_{best}, confs_{accepted})$  \label{alg:mcmc-ga:line:evolve} \\
        $generation \leftarrow generation+1$ \label{alg:mcmc-ga:update_gens}\\
     } \label{alg:mcmc-ga:line:convg}
     \Return{$conf_{best}, perf_{best}$}
\end{algorithm}
%\vspace{-0.25cm}



==> algo_evolve.tex <==
\begin{algorithm}[t!]
    \removelatexerror
\small
  \caption{{The evolutionary sub-routine of EMCMC}}
  \label{alg:evolution}

  \SetKwInOut{Input}{Input} 
   \SetKwInOut{Output}{Output}
   \SetKwRepeat{Do}{do}{while}
   
 \underline{Function Evolve}   \\
  \Input{$conf_{best}, confs_{accepted}$} 
  \Output{$conf_{children}$}
    $conf_{children}$ $\leftarrow$ $EmptyList$ \label{alg:evolve:init_offspring} \\
    $P_{crossover}$ $\leftarrow$ randomly select 50\% parameters from $conf_{best}$ \label{alg:evolve:get_crossover_parameters} \\
    $P_{mutate}$ $\leftarrow$ randomly select 6\% parameters of $conf_{best}$ \label{alg:evolve:get_mutate_parameters}\\
    \ForEach{$conf_p \in confs_{accepted}$} { \label{alg:evolve:iterate_all_parents}
        $conf_{new}$ $\leftarrow$ $crossover(conf_{best}, conf_{p}, P_{crossover})$ \label{alg:evolve:crossover}\\
        $conf_{new}$ $\leftarrow$ $mutate(conf_{new}, P_{mutate})$ \label{alg:evolve:mutate}\\
        $conf_{children}.add(conf_{new})$ \label{alg:evolve:add_into_children}
    }
    \Return{$conf_{children}$} \label{alg:evolve:return}
\end{algorithm}


==> approach.bck.tex <==
\section{Approach}
\label{sect:approach}

Our technical approach to finding good configurations has several parts. First we use problem domain knowledge (here an understanding of Hadoop) to reduce the dimensionality of the space by eliminating  parameters not relevant to the given objective function. In this work we are aiming to improve the performance of the given job, thus, our objective function is CPU time. %: a direct proxy for monetary cost. 

Second, we discretize the space by defining sampling methods for each parameter, varying by parameter type. Boolean parameters are sampled for their true and false values. We sample numerical parameters at a few values less and greater than their defaults. For string-valued parameters (\eg, as Java virtual machine settings) we provide lists of alternative values. 

Third, we undertake an automated meta-heuristic search for high performing configurations in the reduced space. Here, that involves sampling of system configurations, re-configuring a Hadoop cluster to each one, and then profiling the CPU time consumed by the execution of a benchmark-defined map-reduce job under that configuration. We use benchmark-defined {\em small} problem instances (e.g., with several hundred megabytes of input for the word count job type). We run the sampling and benchmarking procedure until a convergence criterion is met or the search budget is exhausted. We return the best configuration found by the search procedure.
\settopmatter{printfolios=true}
\subsection{Framework}
We designed and implemented a software framework, \tool, to drive the search process. We designed it, and we view it, as a demonstration prototype for a framework generalized to work for many software systems, not just Hadoop. To date now we have only used it for the work reported here.

Figure~\ref{fig:framework} illustrates the framework, \tool. It accepts a discretized configuration space model as input. It supports an arbitrary range of metaheuristic search algorithms and can accommodate varying discretization and sampling strategies. In this work, we used two search algorithms: stochastic cyclic coordinate descent and a genetic algorithm. We discuss them in Section~\ref{sect:CD} and ~\ref{sect:GA} respectively.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/framework.png}
    \caption{The framework of configuration exploration with meta-heuristic algorithms}
    \label{fig:framework}
\end{figure}

For Hadoop, our configuration space model is concretely represented as a list of configuration parameters each with a list values to consider in the search, all encoded in a spreadsheet given as input to the framework. We evaluate performance for a given configuration by profiling Hadoop with the HiBench benchmark suite~\cite{huang2010hibench}. We do this for the default configuration, as a baseline, and then iteratively for other configurations produced by the sampling strategy associated with the search algorithm being employed. For each sample, we reconfigure a Hadoop cluster, run a test job, and again measure the CPU time expended. We first prototyped and validated our framework on an in-house, Docker-based Hadoop cluster running on a single multi-CPU server. For the experiments that produced the data we report, we used an Amazon Elastic Map-Reduce (EMR) cluster to assure fidelity to conditions like those an industrial user would face.  

\subsection{Dimensionality Reduction}
\label{sect:reduce-dimension}
We employed three approcahes to reducing the search space. First, we we indicated, we ignored parameters unrelated to our objective function. Second, we discretizing the search space. Third, for one experiment, we measured how each parameter individually influenced performance, and then considered on those with an impact above a certain threshold. Even with this reduction, we obtained positive results. We now further discuss the first and third. 

First, Hadoop has many different types of parameters: to control how to split data into multiple blocks, how much memory to allocate for each map task, names of directories, etc. They provide a rich interface for users to configure Hadoop. Many, however, do not affect the objective function (CPU time). For example, the \textit{hadoop.tmp.dir} parameter defines the temporary base directory and isn't involved in job execution. To reduce the configuration space to only performance related parameters, we use domain knowledge. Hadoop \textit{V2.7.3} has $953$ parameters. We removed most, keeping only $109$.

Second, although some parameters are performance related, they have different levels of impact. We developed a simple heuristic to help us eliminate some variables from consideration. To identify them, we checked how much improvement we could get with respect to the default setting by varying one parameter's value around its default setting. We kept the variables with the greatest effects and cut of those below a somewhat arbitrary threshold, reducing the space from $109$ to $34$ parameters. This approach computes an approximation of the partial derivative of performance with respect each variable in the immediate neighborhood of a reference configuration (here the default value) using the following formula:
$$I_p = \frac{\sum_{i=1}^m \frac{\lvert P_x - P_a \rvert}{P_x}}{m}$$
where $I_p$ is the importance of parameter $p$, $P_x$ is the performance of the reference point $x$, $P_a$ is the performance of an alternative value, and $m$ is the number of alternative values. Suppose the system performance with the default configuration is $100$. A parameter $P$ has $4$ alternative values, and their performance is $[80, 90, 110, 120]$. Then, P's importance is $0.15$. 

We used this technique only in one of our six experiments, involving a word count problem type and a genetic algorithm search technique. We still obtained positive results. We explain this aspect of our experiment for repeatability. We do not claim it as a validated contribution in this paper or as an approach that we expect to work in general. We do plan to repeat the irregular experiment with the full set of $109$ parameters before publication of a final version of this paper.

%first benchmark the system performance with the default configuration. Then we update each individual parameter's value to its available alternatives and benchmark the system for every alternative value. We then computed the {\em uni-dimensional importance of a parameter around the default (or more generally any reference) configuration} with In our prototyping work, we used the resulting ordering of importance of parameters to further reduce the search to about thirty five parameters, cognizant of the shortcomings of this approach (particularly that importance likely varies depending on where one is in the search space). We did not rely on this ordering information to produce the results reported in this paper.
%
%DELETE?
\begin{comment}
\subsection{Coordinate Descent}
\label{sect:CD}
Cyclic coordinate descent~\cite{canutescu2003cyclic-cd} is an iterative, pseudo-gradient descent optimization method in which each iteration of an inner loop optimizes the objective function in one variable only. The next outer loop iterates through the variables. The outermost loop repeats this process until convergence is reached. This algorithm empirically performs reasonably well for many kinds of practical problems. A weakness is that in its innermost loop it does not account for interactions among parameters. Its benefits include being easy to understand and implement; it often converges reasonably quickly; and it admits different optimization strategies for individual parameters.

Algorithm~\ref{alg:coordinate-descent} is the overall procedure of using cyclic coordinate descent to find a better configuration. It accepts a configuration space model and returns the best configuration found. It first gets the initial configuration (line 2) and evaluates it (line 3) to obtain its performance as the current best. The while loop (line 6 - 17) evaluates all parameters one by one. The algorithm will check to see if it is converged after each cycle. If not, another cycle will be started (line 7 - 9). This algorithm shows a stochastic coordinate descent as line 10 randomly sample a next parameter to optimize. Line 18 returns the best found configuration.

\begin{algorithm}[h]
  \caption{Configuration exploration with cyclic\\coordinate descent}
  \label{alg:coordinate-descent}
  \begin{algorithmic}[1]
    \Function{CoordinateDescent}{spaceModel}
        \State{bestConf = getDefaultConf()}
        \State{bestPerf = benchmark(bestConf)}
        \State{allParams = getAllParams()}
        \State{allDirections = allParams}
        \While {not converged()}
            \If{len(allDirections) == 0}
                \State{allDirections = allParams}
            \EndIf
            \State{nextDirec = sample(leftDirections)}
            \State{conf, perf = optimize(nextDirec)}
            \If{perf is better than bestPerf}
                \Let{bestPerf}{perf}
                \Let{bestConf}{conf}
            \EndIf
            \State{allDirections.remove(nextDirec)}
        \EndWhile
        \State \Return{bestConf}
    \EndFunction
  \end{algorithmic}
\end{algorithm}

Algorithm~\ref{alg:single-param-optimize-CD} is the single parameter optimization function that we used in our coordinate descent algorithm. It takes the parameter to be optimized, the current best configuration, and its performance as inputs. Line 3 gets the data type of the input parameter. If it is a numeric variable, like integer or float, the algorithm gets the next alternative value and generates and benchmarks that configuration. It checks whether the new performance is better than the previous best one. If yes, it continues until a new value is found that is not better than the previous best one (Line 4 - 14). If the given parameter is of an enumerated type (boolean, string, etc), this algorithm evaluates all valid values and choose the best one (line 16 - 23). Finally, this function returns the best configuration and corresponding performance. If there is no better value found, this function will just return the input configuration as unchanged.

\begin{algorithm}[h]
  \caption{Optimize individual parameter in cyclic\\coordinate descent}
  \label{alg:single-param-optimize-CD}
  \begin{algorithmic}[1]
    \Require{\textbf{param:} the parameter to optimize.
             \textbf{conf:} current best configuration.
             \textbf{perf:} current best performance.}
    \Ensure{Optimized configuration and its performance}
    \Statex
    \Function{optimizeParam}{param, conf, bestPerf}
        \State{bestV = getCurrValue(param)}
        \State{paramDT = getDataType(param)}
        \If{paramDT is numeric}
            \While{hasNextValue(bestV)}
                \State{nextV = nextValue()}
                \State{nextPerf = benchmark(param, nextV)}
                \If{nextPerf is better than bestPerf}
                    \State{bestPerf = nextPerf}
                    \State{bestV = nextV}
                \Else
                    \State{break}
                \EndIf
            \EndWhile
        \Else
            \State{// parameter is enumerate including bool}
            \State{allValues = getAllValues(param)}
            \State{perfs = benchmark(param, allValues)}
            \State{cBestV, cBestP = getBestV(perfs, allValues)}
            \If{cBestP is better than bestPerf}
                \State{bestPerf = cBestP}
                \State{bestV = cBestV}
            \EndIf
        \EndIf
        \State{conf[param] = bestV}
        \State \Return{conf, bestPerf}
    \EndFunction
  \end{algorithmic}
\end{algorithm}


Algorithm~\ref{alg:CD-convergence} is the convergence check function that we used in our coordinate descent algorithm. Line 2 checks whether a cycle of optimization is done. If not, line 3 returns $False$ indicating that this algorithm has not converge yet. Then line 5 and 6 compute the performance improvement after a cycle is finished. If a configuration found in this cycle improves the performance less than a $threshold$, this function returns $True$ to indicate convergence. Otherwise, $False$ is returned.

\begin{algorithm}[h]
  \caption{Convergence test of cyclic coordinate descent}
  \label{alg:CD-convergence}
  \begin{algorithmic}[1]
    \Statex
    \Function{converged}{preBest, currBest}
        \If{not all parameters optimized}
            \State \Return{False}
        \EndIf
        \State{perfImprovement = preBest - currBest}
        \State{impPercentage = perfImprovement / preBest}
        \If{impPercentage < $threshold$}
            \State \Return{True}
        \EndIf
        \State \Return{False}
    \EndFunction
  \end{algorithmic}
\end{algorithm}
\end{comment}

\subsection{Genetic Algorithm (GA}
\label{sect:GA}
In the context of software configuration spaces, it's known that parameters can interact, thereby defeating naive optimization methods. Meinecke~\cite{meinicke2016complexity} showed that although in practice such interactions are often simpler than the theoretical possibilities, they are often complex enough that it is not possible to reduce search to independent optimization in each dimension, which would effectively make complete analysis feasible.

While coordinate descent is simple and straightforward, it is limited in its capacity to deal with potential interactions among variables. It does not consider them at all within its innermost loop, and it considered them in a limited way only by repeatedly hill-climbing in each dimension until a convergence criterion is satisfied. 

Genetic algorithms~\cite{whitley1994genetic} are meta-heuristic search algorithms that can account for interactions more directly. Such an algorithm starts with $N$ first generation optimization subjects, which are configurations in our case. It measures the quality of these subjects and selects good ones. In the next step, it generates next generation off-spring subjects based on mutation of good parents. It repeats this procedure until a satisfying subject is found or the search budget is exhausted.

Algorithm~\ref{alg:vanilla-genetic} is the algorithm we used to explore a configuration space. Line 3 generates a list of initial first-generation configurations. The while loop from line 7 - 19 iteratively optimizes configurations until convergence or budget depletion is reached. Line 8 measures the performance of all parent configurations. Line 9 and 10 get the best configuration and its performance in this generation. Line 11 - 14 update the global best configuration. Line 16 selects some good parent configurations and line 17 calls the evolution function to create offspring  based on the best configuration and selected good parents.

\begin{algorithm}[h]
  \caption{Genetic algorithm for configuration search}
  \label{alg:vanilla-genetic}
  \begin{algorithmic}[1]
    % \Require{configuration space model}
    % \Ensure{the best configuration found}
    % \Statex
    \Function{Genetic}{spaceModel}
    %   \Let{MAX\_GEN}{50}
    %   \Let{PerfTrack}{empty\_list} \Comment{best performance in each generation}
    %   \Let{InitialConfs}{1000}  \Comment{number of configurations in the first generation}
      \State{MAX\_GEN = K}
      \State{parents = getInitConfs(spaceModel, N)}
      \State{bestConf = None}f
      \State{bestPerf = MAX\_INT}
      \State{gen\_idx = 0}
      \While{gen\_idx $<$ MAX\_GEN}
        \State{perfs = benchmark(parents)}
        \State{currBestC = bestConf(parents, perfs)}
        \State{currBestP = bestPerf(parents, perfs)}
        \If{currBestP is better than bestPerf}
            \State{bestPerf = currBestPerf}
            \State{bestConf = currBestConf}
        \EndIf
        \State{// select configurations to evolve}
        \State{confsToEvolve = selectConfs(parents, perfs)}
        \State{parents = evolve(currBestC, confsToEvolve)}
        \State{gen\_idx += 1}
      \EndWhile
      \State \Return{bestConf}
    \EndFunction
  \end{algorithmic}
\end{algorithm}

Algorithm~\ref{alg:genetic-evolve} is the evolution procedure of our genetic algorithm. It takes the best configuration and selected parent configurations as inputs. There are two main steps in the evolution step: exchange and mutation. Line 3 selects $M$ exchange parameters from all parameters in a configuration. Line 4 selects $N$ mutation parameters from the exchange parameters. For each parent configuration, line 6 exchanges the values of the exchange parameters with those in the best configuration to create a new offspring configuration. Then line 7 randomly mutates values of the mutation parameters in the new configuration. Line 8 adds the newly generated configuration in the offspring set. The entire set offspring configurations are returned in line 10.  

\begin{algorithm}[h]
  \caption{Evolve function in genetic algorithm}
  \label{alg:genetic-evolve}
  \begin{algorithmic}[1]
    % \Require{the best parent configuration and parent configurations}
    % \Ensure{offspring configurations}
    % \Statex
    \Function{evolve}{bestConf, parents}
        \State{offSprings = EmptyList}
        \State{exPs = getExchangeParams($M$)}
        \State{mutatePs = getMutateParams(exPs, $N$)}
        \For{conf in parents}
            \State{newConf = exchangePV(bestConf, conf, exPs)}
            \State{newConf = mutatePV(newConf, mutatePs)}
            \State{offSprings.append(newConf)}
        \EndFor
        \State \Return{offSprings}
    \EndFunction
  \end{algorithmic}
\end{algorithm}

One can define different convergence criteria based on their practical needs and the specific algorithm used to sample the space. In Algorithm~\ref{alg:vanilla-genetic}, the convergence criteria of the genetic algorithm is that the number of generations is larger than a pre-defined maximum threshold. One can also define it in terms of the quality improvement in a generation being less than a threshold, or by combine these two conditions as we do in our case study.

\subsection{Markov Chain Monte Carlo (MCMC)}
Mento Carlo is a sampling method to draw objects from a density distribution $DD(S)$ defined on a high dimensional space $S$. Markov Chain Mento Carlo (MCMC) draws objects in a given space S using a carefully constructed Markov Chain so that high-value regions will be sampled with larger probability. Given a reference point $X$, MCMC draws a neighbor $X^*$ with the proposal distribution and evaluate its fitness value. Then, it decides to accept/reject this neighbor based on the acceptance probability computed based on its fitness value. If a neighbor is accepted, MCMC will transit to it from current state.

In our case, $S$ is the configuration space of a given software system, where the parameters are the dimensions. The proposal distribution is the uniform distribution because we have a discretized configuration space and we randomly select an alternative value for individual parameters. The fitness value is the performance, like CPU time, of a sampled configuration. Whenever a configuration is proposed by the proposal distribution, we dynamically evaluate its performance, compare it with the performance of the reference configuration, and then compute its acceptance probability based on the performance improvement of the sampled configuration.

Like the work of Le et al.\cite{le2015-compiler-mcmc} on finding compiler bugs, we use the exponential function to compute acceptance probability using the following formula:
$$A(C, C^*) = min(1, exp(\sigma*\Delta(P)))$$
, where $C$ is the reference configuration and $C^*$ is the sampled neighbor. $\sigma$ is a constant and $\Delta(P)$ is the performance improvement of $C^*$ over $C$. If the acceptance probability is larger than a random number uniformly sampled from $(0,1)$, the reference point will be updated to this neighbor.

In our implementation, the process of sampling new neighbors is actually realized by the cross-over and mutation operation in genetic algorithms. Given a reference configuration, we sample not only one neighbor but a set of neighbors. Then we evaluate the performance of all neighbors and select those accepted by the algorithm. We update the reference point to the best neighbor. We repeat this process till the pre-defined global performance improvement is achieved or the maximum number of evaluations is met.

If the performance of a configuration is a little bit worse than the reference point, it still has the probability to be accepted. This is one of the main differences compare to GA. In GA, any worse configuration will be discarded. A neighbor is worse than the reference point doesn't mean that it cannot lead to the global optimum.


\subsection{Formalized Configuration Validity Checking}
Configuration parameters have real-world semantic meanings, which are usually documented in an implicit manner. Generally, they exist in places like StackOverflow or Wikipedia. It's easy to make mistakes when configuring a software system without understanding such real-world meanings and constraints, which in return will cause problems like performance degradation and system failures.

In our exploration framework, we use a real-world type checker developed in our previous work to detect potential semantically incorrect configurations generated by our configuration sampling engine. It utilizes Coq's type system to explicitly define real-world types of parameters that are inadequately typed machine types. For example, a buffer size is an integer in machine level. Any integer larger than 0 is a valid value. However, its real-world meaning should be the multiple page size of the underlying hardware. Violation of such semantic constraints could cause performance degradation. In addition to single-parameter constraints, this type checker also define inter-parameters constrains. For example, the maximum heap size of a mapper Java process shouldn't excess 80\% of the total memory allocated to a mapper by Yarn. The other 20\% should be reserved for the code. Such constraints can be added to the checker if found in future. 

Given a configuration, which is a list of <parameter, value> pairs, we first translate it to Coq's representation, and then pass it to the real-world type checker. The checker will call Coq's command-line type checker \textit{coqc} to check the validity of the given configuration. If the configuration fails any checking, the tool will return an error message. Otherwise, no error message is returned and we know the configuration is valid. In our experiments, we evaluate  only valid configurations to save exploration cost.

==> approach_back.tex <==
\section{Technical Approach}
\label{sect:approach}



%To overcome these limitations, we adapt Markov Chain Monte Carlo (MCMC) based sampling strategy. 

%MCMC is a class of sampling algorithms that sample from a high-dimensional space to approximate the target distribution~\cite{chib1995understanding,metropolis1953equation}\textemdash the more samples are drawn, the closer we are to the target distribution. 


 %Usually, MCMC constructs a single Markov Chain that runs for a long time. To help such an MCMC algorithm to converge faster, researchers propose to incorporate features of evolutionary search~\cite{holland1992adaptation} (\eg mutation, cross-over ) in MCMC's sampling strategy~\cite{liang2000evolutionary}. 
 
Our basic approach is to use EMCMC algorithms to sample Hadoop and Spark configuration spaces in search of high-performing configurations. To reduce the cost of, or even need for, costly EMCMC runs, we employ two additional tactics. First, we run Hadoop and Spark using inputs that are several orders of magnitude smaller than those that we want to run in production for sampling performance as a function of configuration. Second, we use a measure of the similarity of big data jobs to enable what amounts to a kind of transfer learning, wherein good configurations for one kind of job are used for another without change. We have implemented our approach in a tool called \tool. This rest of this section describes our approach and technology in detail.

\subsection{Overview}

An overview of \tool is shown in Figure~\ref{fig:framework}. 
\tool takes a big data job as input and outputs a near-optimal configuration by sampling the configuration space using an EMCMC strategy (see Section~\ref{sect:background}).
\tool works in three phases. 
First, in Phase-\rom{1}, it filters out some configuration parameters that are not relevant to the objective function (job performance in our case). 
Next, in Phase-\rom{2}, \tool uses EMCMC sampling strategy to find a near optimal configuration. The sampling process starts
with the default system configuration as the seed value, \ie \tool treats it as the current best configuration at the beginning and then updates it in subsequent steps. While sampling, \tool further discards any invalid configurations that may be generated during sampling using a configuration type-checker that we developed separately (Phase-\rom{3}).  If a configuration is valid, \tool runs a benchmark big data job with this new configuration. \tool records the performance (CPU and wall-clock time) of this execution. It then compares it with that of the currently best configuration, updating the latter if necessary, as per our acceptance criterion (see~\Cref{eq:m}). 
The accepted configurations are subjected to cross-over and mutation to produce the configurations for the next round of sampling.  Once \tool exceeds the sampling budget, it outputs the best configuration found so far. We now describe each of these steps in greater detail.

\begin{figure}[t]
    \centering
    %\includegraphics[width=0.7\textwidth]{figures/framework.pdf}
    \includegraphics[width=0.5\textwidth]{figures/framework.pdf}
    \caption{\textbf{ConEx Workflow}}
    \label{fig:framework}
\vspace{-0.25cm}
\end{figure}


\subsection*{Phase-\rom{1}: Pre-processing the configuration space}  

%A typical configuration space for a big-data framework is high dimensional and complex. 
The total number of configuration parameters for Hadoop and Spark are $901$ and $212$ respectively (see Table~\ref{tab:studied-parameters}). However, the majority are unrelated to performance.
Moreover, not all values of relevant parameters are equally relevant when searching for good results. 

%Further, these parameters can have data types ranging from boolean, integer, float, string, and categorical. 

%Thus, the configuration space forms by varying the total number of potential combinations can be exponentially large. 
%Moreover, multiple parameters usually interact with others. 
%For example, in Hadoop, parameters block size, and minimum data split size together decide how many fragments the input data will be divided into~\footnote{https://wiki.apache.org/hadoop/HowManyMapsAndReduces}.
%Similarly, the number of CPU cores of the resource manager and map/reduce tasks constrain each other, as the total numbers cannot be larger than the number of physical cores. Such diverse data-types and inter-parameter interactions increase the complexity of big-data configuration space significantly. 


The first stage our approach thus reduces the dimensionality of the search space in two ways. First, we consider only relevant parameters, and second, we restrict the sample space by selecting only a few values of each remaining parameter to consider. To select the important features, we use our domain knowledge to remove parameters unrelated to our objective function. We first filter out the parameters that may not influence performance. Although this part is manual, we referred to parameter descriptions by studying technical manuals, as well as a large body of previous work cited in this review paper~\cite{Bonifacio:research_review}. One might argue that manually selecting parameters to study is not reliable and largely reduced the configuration space. However, the configuration space is huge and much larger than those studied in previous work. For example, most subject systems Nair et al.'s paper of rank-based learning approach have only thousands of configurations, with only a few systems like SQLite have millions of configurations. These are just microscopic configuration spaces comparing to the sizes of systems we studied, which are shown in the last column of Table~\ref{tab:studied-parameters}. 

%This manual study took approximately one week for one researcher to complete. How to automate feature selection is an interesting question and will be part of our future work. 

We removed five classes of Hadoop parameters: (i) version related, \eg, \emph{java.runtime.version} and \emph{java.class.version}. These parameters describe the system configuration (\eg Java version ``1.8.0") but have no impact on the CPU time. (ii) file system paths, \eg, \emph{hadoop.bin.path} and \emph{hadoop.log.dir}. Such parameters do not strongly influence computation or CPU time. (iii) authentication related, \eg, \emph{hadoop.http.authentication.kerberos.keytab} and \emph{hadoop.login}. (iv) server-address related, \eg, \emph{mapreduce.jobtracker.http.address}, these parameters are similar to those log directory related parameters. The last class are (v) ID/name related, \eg, \emph{mapreduce.output.basename}, because jobs names do not impact their performance. We reduced the number of parameters from $901$ to $44$.
%Details are in our Github repository.

For Spark, there are $212$ total parameters in version $2.2.0$. They are listed in multiple categories on Spark's website
% \footnote{https://spark.apache.org/docs/2.2.0/configuration.html} 
with detailed explanation. Here we selected parameters that are related to runtime performance wallclock time. Specifically, we selected 27 parameters from \textit{Runtime Environment}, \textit{Shuffle Behavior}, \textit{Compression and Serialization}, \textit{Memory Management}, and \textit{Execution Behavior}, and \textit{Scheduling} categories.

We further discretize the configuration space by defining sampling values for each parameter, varying by parameter type. Boolean parameters are sampled for only true and false values. We sample numerical parameters at a few values less and greater than their defaults. For string-valued parameters (\eg, as Java virtual machine settings) we provide lists of alternative values. 


\subsection*{Phase-\rom{2}: Finding a near-optimal  configuration}

This phase is the core part of our approach,
in which \tool samples the configuration space ($\zeta$) with our EMCMC strategy. 
%As discussed in Section~\ref{sect:background}, it uses an evolutionary version of MCMC algorithm for faster convergence by leveraging cross-over and mutation operations in their sampling strategy. 
Algorithms~\ref{alg:mcmc-ga},~\ref{alg:evolution}, and ~\ref{alg:emcmc-accept} present the constituent routines in detail. 

Algorithm~\ref{alg:mcmc-ga} is the main driving function. Line~\ref{alg:mcmc-ga:line:input} lists the inputs and outputs. This algorithm  samples and evaluates configurations using a given $job$ as a performance benchmark. When complete, it outputs the best configuration that was found, ($conf_{best}$), along with its performance ($perf_{best}$). It takes a configuration as a seed, $conf_{seed}$. It uses two criteria to decide when to terminate and return a result. Either a maximum number of generations, (max\_gen), or a threshold of minimum generation-over-generation performance improvement (min\_improvement) is reached. 

\input{algo_emcmc}

Lines~\ref{alg:mcmc-ga:line:init_perf} to~\ref{alg:mcmc-ga:init_global_imp} initialize some parameters including setting the best configuration and performance to the respective seed values.  Line~\ref{alg:mcmc-ga:line:sample_fst_generation} gets the first generation of configurations by randomly sampling $n$ items from the configuration space $\zeta$. We choose $n=200$, but it could be set to any reasonable value. Line~\ref{alg:mcmc-ga:line:loop_start} to \ref{alg:mcmc-ga:line:loop_end} are the main procedure for evaluating and evolving \wrt each configuration. Given a configuration $conf_p$, Line~\ref{alg:mcmc-ga:line:loop_start} records the job's performance ($perf_p$) and line~\ref{alg:mcmc-ga:line:accept} decides whether to accept it based on equation~\ref{eq:m}. This part is realized in Algorithm~\ref{alg:emcmc-accept}. If accepted, Line~\ref{alg:mcmc-ga:line:add_accepted} stores the accepted configuration to a list $confs_{accepted}$. This list is used in generating next-generation configurations (line~\ref{alg:mcmc-ga:line:evolve}). Line~\ref{alg:mcmc-ga:line:update_best_start} to~\ref{alg:mcmc-ga:line:update_best_end} update the previously found best configuration and best performance if the accepted one is better. 

Once all the first generation configurations are processed, line~\ref{alg:mcmc-ga:update_global_imp} computes the performance improvement achieved by the first generation \wrt the seed performance, which is our baseline. Next at line~\ref{alg:mcmc-ga:line:evolve}, the algorithm prepares to enter the next generation by generating offspring configurations using cross-over and mutation operations (see Algorithm~\ref{alg:evolution}). Line~\ref{alg:mcmc-ga:update_gens} updates the generation number. This process repeats until a termination criterion is satisfied (line~\ref{alg:mcmc-ga:line:convg}). The last line returns the best found configuration and the corresponding performance.

Algorithm~\ref{alg:evolution} is the evolution sub-routine of the our EMCMC algorithm. It is adapted from a standard Genetic Algorithm~\cite{holland1992adaptation}. For preparing configurations of the next generation, it takes the best configuration found so far and a list of parent configurations as inputs. There are two main steps in the evolution process: cross-over and mutation. From the best configuration, Line~\ref{alg:evolve:get_crossover_parameters} selects half of all parameters as cross-over parameters ($P_{crossover}$), and Line~\ref{alg:evolve:get_mutate_parameters} identifies 6\% of them as mutation parameters ($P_{mutate}$). Next, for each parent configuration, line~\ref{alg:evolve:crossover} exchanges the values of the cross-over parameters with $P_{crossover}$. It then randomly mutates the values of the mutation parameters at line~\ref{alg:evolve:mutate} . The resulting offspring is added into the children set at line~\ref{alg:evolve:add_into_children}. A set of new offspring configurations is returned at line~\ref{alg:evolve:return}.  

\input{algo_evolve}

Algorithm~\ref{alg:emcmc-accept} is the function to compute acceptance probabilities. It takes the performance of the current best configuration and that of the current candidate as inputs and returns whether to accept/reject the candidate. Line~\ref{alg:emcmc-accept:compute_imp} computes the performance improvement as $\Delta perf$. For example, $\Delta perf$ can be $0.01$ or $-0.02$ indicating percentage performance improvement. If the current configuration is worse than the best value, the result will be negative. Line~\ref{alg:emcmc-accept:compute_acc_prob} computes the acceptance probability of the configuration using an exponential function. This function returns a positive value even if $\Delta perf$ is negative. Finally, the acceptance probability is compared with a random number sampled between $0$ and $1$. Thus, even if a configuration is slightly worse than the best one, it still has some chance of being accepted.

\begin{algorithm}[h]
\scriptsize
  \caption{{Accept function of EMCMC}}
  \label{alg:emcmc-accept}

  \SetKwInOut{Input}{Input} 
   \SetKwInOut{Output}{Output}
   \SetKwRepeat{Do}{do}{while}
   
 \underline{Function Accept}   \\
  \Input{$perf_{best}, perf_{p}$} 
  \Output{bool: accept/reject $conf_p$}
     
    $\Delta perf$ $\leftarrow$ $\frac{perf_{best} - perf_{p}}{perf_{best}}$ \label{alg:emcmc-accept:compute_imp} \\
    $accept\_prob$ $\leftarrow$ $exp(50*\Delta perf)$ \label{alg:emcmc-accept:compute_acc_prob}\\
    \If{$Rand(0, 1) < accept\_prob$} {  \label{alg:emcmc-accept:compare_with_rand}
	    \Return{True}
    }
    \Return{False}
\end{algorithm}


\subsection*{Phase-\rom{3}: Configuration Validity Checking}
Configuration spaces are often not complete cross-product spaces. Rather, they are subsets defined by constraints on individual parameter values and sets of parameter values. A problem that we encountered is that  constraints on configurations---at least for Hadoop and Spark, and we expect for many systems---are not well documented, nor statically enforced. One might have to search developer web sites to find all relevant constraints, or even just run systems to find out whether configurations cause malfunctions. Indeed, even the types of fields are often not very well specified. For example, the type of Hadoop's \textit{JVM options} parameter is \textit{string}, but not any string will do. The lack of documentation of types (constraints) and enforcement makes it not only easy to make configuration errors, but also also vastly increases search space sizes. 

To reduce the search space our tool had to consider, and to mitigate the possibility of returning an ill-formed configuration, in previous work we developed, and in this system we used, a \textit{real-world type checker for configurations}~\cite{tang2017interpreted}. It allows for the imposition of constraints on fields and sets of fields, taking advantage of Coq's expressive logic~\cite{barras1997coq} to encode, and its type checker to enforce,  constraints. Further details are beyond the scope of this work. Suffice it to say that checking the known constraints allowed us to avoid costly dynamic evaluation of about 8\% of all of the configurations that our approach sampled, as judged by results of some of our Hadoop runs. 

%type system to explicitly define real-world types of parameters that are inadequately typed machine types. For example, a buffer size is an integer in machine level. Any integer larger than 0 is a valid value. However, its real-world meaning should be the multiple page size of the underlying hardware. Violation of such semantic constraints could cause performance degradation. In addition to single-parameter constraints, this type checker also defines inter-parameters constraints. For example, the maximum heap size of a mapper Java process should not excess 80\% of the total memory allocated to a mapper by Yarn. The other 20\% should be reserved for the code. Such constraints can be added to the checker if found in future. Given a configuration, which is a list of <$parameter, value$> pairs, we first translate it to Coq's representation and then pass it to the real-world type checker. The checker calls Coq's command-line type checker \textit{coqc} to check the validity of the given configuration. If the configuration fails any checking, the tool returns an error. Otherwise, the configuration passes the type checking and is valid. In our experiments, we explore with only valid configurations to save the exploration cost.


% This is redundant to some section in Experiment section
% \subsection{Multi-Resolution Exploration}
% Due to the big-data nature of data processing infrastructures, the exploration cost could be too high for an organization to afford. Therefore, we propose this multi-resolution approach to first explore the whole configuration space with small job instance. Once we found some good configurations, we evaluate them with larger (10X and 100X) job instances to further pick out better configurations. Using small job instance to explore the whole configuration space can save a large amount of cost, but it could lead to some \textit{not-so-good} configurations. This multi-resolution can avoid such glitches by adding post-processing steps to the exploration phase.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The following content is commented out.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
\subsubsection{Genetic Algorithm (GA)} 
\label{sect:GA}
Other than learning-based and random sampling approaches, we utilize meta-heuristic search methods to explore a configuration space. Genetic algorithms are well-known in optimizing functions of discrete variables. In our representation, configuration space is discretized, such that we can leverage GAs to optimize it. 

GAs are meta-heuristic search algorithms~\cite{whitley1994genetic} that can account for parameter interactions more directly. Such an algorithm starts with $N$ first generation optimization subjects, which are configurations in our case. It measures the quality of these subjects and selects good ones. In the next step, it generates next generation off-spring subjects based on mutation of good parents. It repeats this procedure until a satisfying subject is found or the search budget is exhausted.

Algorithm~\ref{alg:vanilla-genetic} is the algorithm we used to explore a configuration space. Line 3 generates a list of initial first-generation configurations. The while loop from line 7 - 19 iteratively optimizes configurations until convergence or budget depletion is reached. Line 8 measures the performance of all parent configurations. Line 9 and 10 get the best configuration and its performance in this generation. Line 11 - 14 update the global best configuration. Line 16 selects some good parent configurations and line 17 calls the evolution function to create offspring  based on the best configuration and selected good parents.

\begin{algorithm}[h]
  \caption{Genetic algorithm for configuration search}
  \label{alg:vanilla-genetic}
  \begin{algorithmic}[1]
    % \Require{configuration space model}
    % \Ensure{the best configuration found}
    % \Statex
    \Function{Genetic}{spaceModel}
    %   \Let{MAX\_GEN}{50}
    %   \Let{PerfTrack}{empty\_list} \Comment{best performance in each generation}
    %   \Let{InitialConfs}{1000}  \Comment{number of configurations in the first generation}
      \State{MAX\_GEN = K}
      \State{parents = getInitConfs(spaceModel, N)}
      \State{bestConf = None}f
      \State{bestPerf = MAX\_INT}
      \State{gen\_idx = 0}
      \While{gen\_idx $<$ MAX\_GEN}
        \State{perfs = benchmark(parents)}
        \State{currBestC = bestConf(parents, perfs)}
        \State{currBestP = bestPerf(parents, perfs)}
        \If{currBestP is better than bestPerf}
            \State{bestPerf = currBestPerf}
            \State{bestConf = currBestConf}
        \EndIf
        \State{// select configurations to evolve}
        \State{confsToEvolve = selectConfs(parents, perfs)}
        \State{parents = evolve(currBestC, confsToEvolve)}
        \State{gen\_idx += 1}
      \EndWhile
      \State \Return{bestConf}
    \EndFunction
  \end{algorithmic}
\end{algorithm}

One can define different convergence criteria based on their practical needs and the specific algorithm used to sample the space. In Algorithm~\ref{alg:vanilla-genetic}, the convergence criteria of the genetic algorithm is that the number of generations is larger than a pre-defined maximum threshold. One can also define it in terms of the quality improvement in a generation being less than a threshold, or by combine these two conditions as we do in our case study.
\end{comment}


\begin{comment}
\subsection{Dimensionality Reduction}
\label{sect:reduce-dimension}
We employed three approahes to reducing the search space. First, we we indicated, we ignored parameters unrelated to our objective function. Second, we discretizing the search space. Third, for one experiment, we measured how each parameter individually influenced performance, and then considered on those with an impact above a certain threshold. Even with this reduction, we obtained positive results. We now further discuss the first and third. 

First, Hadoop has many different types of parameters: to control how to split data into multiple blocks, how much memory to allocate for each map task, names of directories, etc. They provide a rich interface for users to configure Hadoop. Many, however, do not affect the objective function (CPU time). For example, the \textit{hadoop.tmp.dir} parameter defines the temporary base directory and isn't involved in job execution. To reduce the configuration space to only performance related parameters, we use domain knowledge. Hadoop \textit{V2.7.3} has $953$ parameters. We removed most, keeping only $109$.

Second, although some parameters are performance related, they have different levels of impact. We developed a simple heuristic to help us eliminate some variables from consideration. To identify them, we checked how much improvement we could get with respect to the default setting by varying one parameter's value around its default setting. We kept the variables with the greatest effects and cut of those below a somewhat arbitrary threshold, reducing the space from $109$ to $34$ parameters. This approach computes an approximation of the partial derivative of performance with respect each variable in the immediate neighborhood of a reference configuration (here the default value) using the following formula:
$$I_p = \frac{\sum_{i=1}^m \frac{\lvert P_x - P_a \rvert}{P_x}}{m}$$
where $I_p$ is the importance of parameter $p$, $P_x$ is the performance of the reference point $x$, $P_a$ is the performance of an alternative value, and $m$ is the number of alternative values. Suppose the system performance with the default configuration is $100$. A parameter $P$ has $4$ alternative values, and their performance is $[80, 90, 110, 120]$. Then, P's importance is $0.15$. 

We used this technique only in one of our six experiments, involving a word count problem type and a genetic algorithm search technique. We still obtained positive results. We explain this aspect of our experiment for repeatability. We do not claim it as a validated contribution in this paper or as an approach that we expect to work in general. We do plan to repeat the irregular experiment with the full set of $109$ parameters before publication of a final version of this paper.

%first benchmark the system performance with the default configuration. Then we update each individual parameter's value to its available alternatives and benchmark the system for every alternative value. We then computed the {\em uni-dimensional importance of a parameter around the default (or more generally any reference) configuration} with In our prototyping work, we used the resulting ordering of importance of parameters to further reduce the search to about thirty five parameters, cognizant of the shortcomings of this approach (particularly that importance likely varies depending on where one is in the search space). We did not rely on this ordering information to produce the results reported in this paper.
%
%DELETE?

\subsection{Coordinate Descent}
\label{sect:CD}
Cyclic coordinate descent~\cite{canutescu2003cyclic-cd} is an iterative, pseudo-gradient descent optimization method in which each iteration of an inner loop optimizes the objective function in one variable only. The next outer loop iterates through the variables. The outermost loop repeats this process until convergence is reached. This algorithm empirically performs reasonably well for many kinds of practical problems. A weakness is that in its innermost loop it does not account for interactions among parameters. Its benefits include being easy to understand and implement; it often converges reasonably quickly; and it admits different optimization strategies for individual parameters.

Algorithm~\ref{alg:coordinate-descent} is the overall procedure of using cyclic coordinate descent to find a better configuration. It accepts a configuration space model and returns the best configuration found. It first gets the initial configuration (line 2) and evaluates it (line 3) to obtain its performance as the current best. The while loop (line 6 - 17) evaluates all parameters one by one. The algorithm will check to see if it is converged after each cycle. If not, another cycle will be started (line 7 - 9). This algorithm shows a stochastic coordinate descent as line 10 randomly sample a next parameter to optimize. Line 18 returns the best found configuration.

\begin{algorithm}[h]
  \caption{Configuration exploration with cyclic\\coordinate descent}
  \label{alg:coordinate-descent}
  \begin{algorithmic}[1]
    \Function{CoordinateDescent}{spaceModel}
        \State{bestConf = getDefaultConf()}
        \State{bestPerf = benchmark(bestConf)}
        \State{allParams = getAllParams()}
        \State{allDirections = allParams}
        \While {not converged()}
            \If{len(allDirections) == 0}
                \State{allDirections = allParams}
            \EndIf
            \State{nextDirec = sample(leftDirections)}
            \State{conf, perf = optimize(nextDirec)}
            \If{perf is better than bestPerf}
                \Let{bestPerf}{perf}
                \Let{bestConf}{conf}
            \EndIf
            \State{allDirections.remove(nextDirec)}
        \EndWhile
        \State \Return{bestConf}
    \EndFunction
  \end{algorithmic}
\end{algorithm}

Algorithm~\ref{alg:single-param-optimize-CD} is the single parameter optimization function that we used in our coordinate descent algorithm. It takes the parameter to be optimized, the current best configuration, and its performance as inputs. Line 3 gets the data type of the input parameter. If it is a numeric variable, like integer or float, the algorithm gets the next alternative value and generates and benchmarks that configuration. It checks whether the new performance is better than the previous best one. If yes, it continues until a new value is found that is not better than the previous best one (Line 4 - 14). If the given parameter is of an enumerated type (boolean, string, etc), this algorithm evaluates all valid values and choose the best one (line 16 - 23). Finally, this function returns the best configuration and corresponding performance. If there is no better value found, this function will just return the input configuration as unchanged.

\begin{algorithm}[h]
  \caption{Optimize individual parameter in cyclic\\coordinate descent}
  \label{alg:single-param-optimize-CD}
  \begin{algorithmic}[1]
    \Require{\textbf{param:} the parameter to optimize.
             \textbf{conf:} current best configuration.
             \textbf{perf:} current best performance.}
    \Ensure{Optimized configuration and its performance}
    \Statex
    \Function{optimizeParam}{param, conf, bestPerf}
        \State{bestV = getCurrValue(param)}
        \State{paramDT = getDataType(param)}
        \If{paramDT is numeric}
            \While{hasNextValue(bestV)}
                \State{nextV = nextValue()}
                \State{nextPerf = benchmark(param, nextV)}
                \If{nextPerf is better than bestPerf}
                    \State{bestPerf = nextPerf}
                    \State{bestV = nextV}
                \Else
                    \State{break}
                \EndIf
            \EndWhile
        \Else
            \State{// parameter is enumerate including bool}
            \State{allValues = getAllValues(param)}
            \State{perfs = benchmark(param, allValues)}
            \State{cBestV, cBestP = getBestV(perfs, allValues)}
            \If{cBestP is better than bestPerf}
                \State{bestPerf = cBestP}
                \State{bestV = cBestV}
            \EndIf
        \EndIf
        \State{conf[param] = bestV}
        \State \Return{conf, bestPerf}
    \EndFunction
  \end{algorithmic}
\end{algorithm}


Algorithm~\ref{alg:CD-convergence} is the convergence check function that we used in our coordinate descent algorithm. Line 2 checks whether a cycle of optimization is done. If not, line 3 returns $False$ indicating that this algorithm has not converge yet. Then line 5 and 6 compute the performance improvement after a cycle is finished. If a configuration found in this cycle improves the performance less than a $threshold$, this function returns $True$ to indicate convergence. Otherwise, $False$ is returned.

\begin{algorithm}[h]
  \caption{Convergence test of cyclic coordinate descent}
  \label{alg:CD-convergence}
  \begin{algorithmic}[1]
    \Statex
    \Function{converged}{preBest, currBest}
        \If{not all parameters optimized}
            \State \Return{False}
        \EndIf
        \State{perfImprovement = preBest - currBest}
        \State{impPercentage = perfImprovement / preBest}
        \If{impPercentage < $threshold$}
            \State \Return{True}
        \EndIf
        \State \Return{False}
    \EndFunction
  \end{algorithmic}
\end{algorithm}

\end{comment}


% already covered in Phase-II, so comment out
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
We designed and implemented a software framework, \tool, to drive the search process. We designed it, and we view it as a demonstration prototype for a framework generalized to work for many software systems, not just Hadoop. To date now we have only used it for the work reported here. Figure \ref{fig:framework} illustrates the framework, \tool, with MCMC as the search algorithm. It accepts a discretized configuration space model as input. It supports an arbitrary range of metaheuristic search algorithms and can accommodate varying discretization and sampling strategies. In this work, we mainly use the MCMC algorithm, which we will discuss it in detail in Section~\ref{sect:mhs}. 

The framework first take the given reference configuration, the default configuration in~\ref{fig:framework}, as the best one. Then, the sampling strategy (MCMC sampling in the figure) samples a set of configurations samples and feed them to the \textit{Evaluator}. The \text{acceptance checker} will decide whether to accept a configuration. The best configuration will be updated if the current one is better than it. Then the accepted configuration will be feed into the sampling strategy to create the next configuration. The whole procedure will exit if the predefined stop criterion is met.

For Hadoop, our configuration space model is concretely represented as a list of configuration parameters each with a list values to consider in the search, all encoded in a spreadsheet given as input to the framework. We evaluate performance for a given configuration by profiling Hadoop with the HiBench benchmark suite~\cite{huang2010hibench}. We do this for the default configuration, as a baseline, and then iteratively for other configurations produced by the sampling strategy associated with the search algorithm being employed. For each sample, we reconfigure a Hadoop cluster, run a test job, and again measure the CPU time expended.
\end{comment}


==> experiment_bck.tex <==
\section{Experimental Design}
\label{sect:experiment}

%In this section, we discuss the implementation of \tool, the subject systems we studied, and our experimental design. 
We implement \tool with Python with about $4000$ lines of code. 
%To support transparency, data and software retention, artifact evaluation, and independent evaluation and repeatability of our experiments, we make our implementation 
It is available in a public Github repository: \url{https://www.github.com/username/blind}.



\subsection{Study Subject} 
We applied our approach to Hadoop
%~\footnote{\url{http://hadoop.apache.org}} 
and Spark~\cite{zaharia2010spark}. 
We developed our methodology by focusing on Hadoop and then validating it using Spark. Hadoop and its variants and extensions are the most widely used systems for big data computing today. Spark is another similarly popular big data framework. The main difference is that it utilizes memory as much as possible in lieu of mass storage to reduce execution times. %We used Apache Spark version \textit{2.2.0}. 

%Hadoop's $900+$ parameters are spread in four configuration files (CORE, HDFS, MAPREDUCE, and YARN). There are clearly interactions among some of these parameters. For example, the settings of block size and minimum data split size together decide the number of fragments the input data will be divided into~\footnote{https://wiki.apache.org/hadoop/HowManyMapsAndReduces}. The number of CPU cores of resource manager and map/reduce tasks constrain each other, as the total numbers cannot be larger than the physical cores. 


Table~\ref{tab:studied-parameters} summarizes the parameters we studied for Hadoop $v2.7.4$ and Spark $v2.2.0$. 
%It lists the total number of parameters in each system, among which how many we studied in this work, as well as how many parameters there are in each data type.
%Table~\ref{tab:studied-parameters} shows the studied configuration spaces for both the frameworks. 
Hadoop has $901$ parameters  across four sub-systems (CORE, HDFS, MAPREDUCE, and YARN) with diverse types.  After preprocessing (Phase-\rom{1}), we identified 44 parameters relevant to performance. 
%Of them, 4 are boolean, 26 are integer, 6 are float,  3  are categorical, and 5 are of type string. 
Similarly, out of 212 Spark parameters,  27 of different types were relevant. Thus, total we studied $3*10^{28}$ and $4*10^{16}$ parameters. Such configuration space is order of magnitude larger and complex than the configuration space  studied before~\cite{nair-bad-learners}. To further reduce the space, we select $\pm 10$\% values around the default for numeric values and all the possible values for boolean and categorical types.

%For booleans, the values are \textit{[True, False]}. For categorical parameters, we take values from official documentation. For numeric parameters, we define two smaller and two larger values around the default, with a $\Delta$ of 10\%. If a parameter default value is $100$, the $\Delta$ will be $10$ and the  alternative values will be $[80, 90, 110, 120]$. Some numeric parameters have $0$ as their default values. In this case, we refer the official documents to define a list of alternative values that respect its semantic meaning.
 
%We represent a discretized configuration space as a list of \textit{<parameter, list<values>>} pairs. 
% In Phase-\rom{2}, we sampled and generated parameter values. For booleans, the values are \textit{[True, False]}. For categorical parameters, we take values from official documentation. For numeric parameters, we define two smaller and two larger values around the default, with a $\Delta$ of 10\%. If a parameter default value is $100$, the $\Delta$ will be $10$ and the  alternative values will be $[80, 90, 110, 120]$. Some numeric parameters have $0$ as their default values. In this case, we refer the official documents to define a list of alternative values that respect its semantic meaning. 

% We do not claim that this sampling strategy is optimal. We leave the design and evaluation of more sophisticated strategies for future work. Suffice it to say that even this simple strategy produced significant positive results, suggesting that there is even more potential performance to be recovers in the future. In future work we plan to generalize our framework to use semantically informed sampling, using constraint-based sampling, sampling from distributions that justified using domain knowledge, etc.

%User-created Hadoop configurations are stored in four \textit{.xml} files in the \textit{\$HADOOP\_HOME/etc/hadoop} directory: \textit{core-site.xml}, \textit{mapred-site.xml}, \textit{hdfs-site.xml}, and \textit{yarn-site.xml}. 
% Once \tool sample and generate a new configuration in Phase-\rom{2} of Section~\ref{sect:approach},  four new \textit{.xml} files are created and stored in Hadoop's configuration folders. \tool then restarts Hadoop to make the new configuration effective.
% ~\chong{what happens for Spark?}

We conducted our experiments in our in-house Hadoop and Spark clusters, which have one master node and four slave nodes. Each node has a Intel(R) Xeon(R) E5-2660 CPU and 32GB memory. We assigned 20GB for Hadoop on each node in our experiments. We also made sure that no other programs were running except core Linux OS processes.

\subsection{Benchmark Tool}
%Hadoop supports multiple types of map-reduce jobs: information extraction from large sets of data, machine learning, web indexing, and so on. These jobs usually have different requirements for software configurations. We settled on a core Hadoop installation without any add-on or alternative components. We were thus limited to certain job types available in the HiBench suite. 

HiBench~\cite{huang2010hibench} is a benchmark suite for big data framework evaluation. It provides benchmark jobs for both Hadoop and Spark. For Hadoop, we selected five jobs: WordCount, Sort, TeraSort, PageRank, and NutchIndex from the \textit{Micro} and \textit{Websearch} categories. These jobs only need a core Hadoop system to execute as opposed to other categories that require Hive or Spark. For Spark, we selected five jobs: WordCount, Sort, TeraSort, RF, and SVD. In this case, WordCount, Sort, and Terasort are Spark implementations that are different from the Hadoop jobs.

% The job types we selected are listed as follows.
% \begin{itemize}
%     \item \textbf{WordCount} This job counts the number of appearance of words in the input data.
%     \item \textbf{Sort} This job sorts text in the input data.
%     \item \textbf{TeraSort} This job is a MapReduce implementation of the standard benchmark created by Jim Gray~\cite{gray1998sort}. 
% \end{itemize}

HiBench defines six different sizes of input workload, from ``tiny'' to ``Bigdata''.
% For example, the different levels of inputs of \textit{WordCount}, including their names and sizes, are listed in Table~\ref{tab:hibench-datasize}. 
To vastly reduce the cost of sampling, we mainly use ``small'' data inputs. To validate the underlying hypothesis that results obtained in this manner will still produce improved performance at scales several orders of magnitude greater, we then benchmark the same jobs on the synthesized configurations using ``large'' and ``huge'' data inputs. 

% \begin{table}[h]
% % \setlength{\tabcolsep}{1.5pt}
% \renewcommand{\arraystretch}{1.5}
% \scriptsize
% \centering
% \caption{Input data sizes for \textit{Micro} jobs in HiBench}
% \label{tab:hibench-datasize}
% \begin{tabular}{c|c|c|c|c|c}
% \hline
% \textbf{Tiny} & \textbf{Small} & \textbf{Large} & \textbf{Huge} & \textbf{Gigantic} & \textbf{Bigdata} \\ 
% \hline
% 32KB & 320MB & 3.2GB & 32GB & 320GB    & 3.2TB   \\ 
% \hline
% \end{tabular}
% \end{table}



\subsection{\tool Settings}

For each generation, as a heuristic, we generate around $4D$ samples, where $D$ is the number of parameters. It is common in applications using GA techniques to set the next population size at $2D$. We set the  maximum number of generations to $30$. Our cross-over step randomly exchanges the values of half of the parameters. Our mutation step randomly selects 6\% of all parameter and mutates their values. We have already explained our termination criteria. 

\subsection{Job Classification}
To further reduce the cost of sampling, and indeed to avoid it altogether in some cases, we hypothesized that configurations found to be good for one kind of job might also work well for other, similar kinds of jobs. To test this {\em scale-out} hypothesis we needed a way to cluster jobs by similarity. HiBench classifies jobs by their business purposes. For example, it classifies all web page indexing and ranking related jobs in the \textit{Websearch} category. However, such a classification does not necessarily reflect the computational characteristics of a jobs. We thus developed and evaluated an approach to clustering jobs by profiling their run-time behaviors based on system call traces. This approach has been widely used in security community~\cite{khadke2012transparent, yoon2014toward, kasick2009system}.

\textit{strace}, a Unix command line tool for capturing system calls of a process, provides rich information about how processes use system resources. The typical application scenario is to capture system calls of a process on a single machine. However, Hadoop and Spark run on multiple machines. Luckily, both of them can be configured to run a single machine. In this mode, a task runs as a single Java process. In this work, we configure Hadoop and Spark in the single-node mode so that we can capture a job's system calls. Then, we compute the similarity of jobs based on the gathered logs.

We represent a job as four parts: 1) the call sequence, 2) the term frequency of string and categorical arguments, 3) the unique term sets of string and categorical arguments, and 4) the mean value of numerical arguments. Each part is a sub-similarity that contributes to the overall similarity. To compute the similarity of two jobs, we first compute the similarity of these four parts and then take the average value of these sub-similarities to compute the overall similarity, which means that each part has the same weight. 

To compute call sequence similarity, we used pattern matching to compute the similarity of their sub-sequences, where each call sequence is sliced into many sub-sequences. To compute term frequency similarity, we compute the average difference of each term frequency. To compute the similarity of unique term sets, we compute the Jaccard Index, which is a common approach to compute the similarity of two sets. We compute the similarity of mean value of numerical arguments as $1 - abs(mean1, mean2)/max(mean1, mean2)$.


\subsection{Sensitivity Analysis}
\label{sect:sensitivity}
To understand how much a parameter contributes to performance improvement, we conduct sensitivity analysis for each synthesized configuration. Given a job, we measure its performance under the default and best configurations found by \tool: $perf_d$ and $perf_b$. We compute the best performance improvement as $imp_b = (perf_d - perf_b)/perf_d$. Based on the best configuration, we create a new configuration by setting each parameter in turn back to its default and measuring the performance, $perf_n$. The performance improvement of this new configuration is defined as $imp_n = (perf_d - perf_n)/perf_d$. The sensitivity of a parameter is then the difference of performance improvement, $sensitivity = imp_b - imp_n$. We conduct this analysis for all Hadoop jobs. We discuss detailed results in Section~\ref{sect:results}.

\subsection{Comparing with Learning-based Approach}
Many previous work solves the problem of finding high-performing configurations with learning-based approaches. In this line of work, researchers first gather system usage data to train a prediction model, and then use this model to find good configurations. While most work tries to build high-accuracy models, Nair et al.~\cite{nair-bad-learners} argue that a model that can preserve configuration ranking is enough to find good configurations. They compared their rank-based models with residual-based models and demonstrated that a rank-based model has the same or higher effectiveness in finding high-performing configurations.

In this work, we compare our approach that based on meta-heuristics search algorithms with the work of Nair et al., to find out which approach is more effective in finding high-performing configurations. We adopt the same criterion used in their paper: the rank-difference of configurations.


==> intro.bak.tex <==
\section{Introduction}
\label{sect:introduction}

Configuring systems with high-dimensional, complex configuration spaces to perform well is hard. Users often end up just using pre-packaged default configurations provided with such systems. We present apparatus, experimental designs, and experimental results that suggest that direct metaheuristic search for high-performing configurations has the potential to cost-effectively find configurations that perform much better than baseline default configurations. We also present experimental results supporting an approach to significantly reducing the cost of search, wherein we evaluate the performance of given configurations using small problem instances in the expectation that the resulting configurations might also work well on the much larger problem instances likely to be important in production work.

\subsection{Problem}
Many important software systems are highly configurable and, at least in principle, can be tailored to meet different needs in different environments and to perform well when doing so. In practice, people often find it hard to understand how to take advantage of these rich degrees of configurability, and so they often just accept the default configurations, leaving significant performance improvement potential unrealized. New methods are needed to help users find high-performing configurations for such systems.

The problem has several major, well studied aspects, and some that are not yet as well studied. Among them are the following. First, the kind of configuration spaces in question are vast, with multiple values possible for each of dozens or hundreds of parameters. Second, configurations are often not just flat vectors of numerical values, as in typical optimization problems, but rather are complex data structures, with fields of multiple types, and often, we observe, with dependent substructures, e.g., where one parameter being set to {\em true} enables some subsystem, requiring that additional values be provided for that subsystem. Standard mathematical methods for optimizing numerical objective functions don't apply. Third, these configuration spaces are also often not just cross-products of their constituent parameter values, but are subject to additional constraints. Fourth, these spaces can be parameterized by external values: e.g., one cannot set  number-of-CPUs (a constraint) to a number larger than the number of CPUs in the system in question (the external parameter). Fifth, analysts often don't know key properties of configuration-to-performance functions: e.g., how parameters interact, whether properties analogous to convexity and linearity apply, etc. Sixth, one usually lacks mathematical performance objective functions that are easy to evaluate, and so one is stuck with having to compute the function for each configuration by actually running and profiling the system under the given configuration. This is generally expensive and gives rise to the need for ways to find good configurations without having to compute the objective function too many times.  

\subsection{State of the Art} 
The problem of finding high-performing system designs and configurations has given rise to a significant body of work. This work both explicates the nature of the problem and proposes methods to address it.
% I think we can remove the Arcuri paper from here. They studied the effect of parameter tuning for search algorithms themselves, but not the system parameters.
%Arcuri et al.~\cite{arcuri2013parameter}, for example, working in the particular problem domain of test data generation, for example, presented results of extensive experimentation suggesting that searching for good configurations is a costly proposition and in practice just using default parameter settings is a reasonable choice. Much work nevertheless continues on ways to find better configurations, across a broad range of system and problem types. 
Much current state of the art work focuses on learning inexpensive-to-evaluate predictive models for mapping arbitrary configuration states to sufficiently accurate estimated performance outcomes, and on then using these models in model-based search approaches to find good configurations cost effectively. To learn models, however, one must profile a system under varying configuration conditions and then generalize from the resulting samples. Profiling systems is generally costly, so the challenge is to learn suitable models with as few profiling runs (evaluations of the actual objective function) as possible.

Siegmond et al. focus on reducing the cost to learn accurate predictive models in the presence of configuration feature interactions~\cite{siegmund2012predictperf, siegmund2015performance}. Nair et al.~\cite{nair-bad-learners} aim to reduce the cost of learning by relaxing the requirement for accurate predictions of performance to one for accurate {\em ordering} by performance. Zhang et al.~\cite{zhang2015performance} assume all parameters are boolean variables and thus formulate the performance prediction problem as learning the Fourier coefficients of boolean functions. Venkataraman et al.~\cite{venkataraman2016ernest} aim to predict performance for jobs running on a shared cloud infrastructure. They learn a performance model from previous runs of small instances to predict performance for larger instances.

% However, configuration parameters give rise to spaces where a huge number of configurations with different run-time performance exist. Such spaces are generally highly-nonlinear and perhaps non-convex. Although tuning a configurable system is relatively easy, understanding and efficiently optimizing the consequent performance is costly and error-prone. A previous work~\cite{ren2013hadoop} shows that, in the Hadoop community, users just accept the default settings most of the time. In this paper, we aim to find good configurations for such complex and high-dimension systems with meta-heuristic search algorithms.

% A configuration space is imaginable huge because the large number of parameters in a system and each one of them could have multiple possible values. Suppose a system has $N$ parameters and each one has $M$ values on average, the theoretical number of configurations is $M^N$ in this case. Although the real number could be much smaller in practice, it is still intractable to find a good configuration. For example, there are more than 900 parameters in Hadoop \textit{V2.7.3}. Such large number of parameters enable users to tailor almost every piece of the software, but it also produces many difficulties to do so due to potential unknown consequences of adjusting them.

%Besides the large number of parameters exist in a system. They often collaboratively control a system to carry out user jobs and constrain each other. Such inter-parameter interactions create more difficulties in system tuning. The logical types of configuration spaces, defining valid configuration settings, can be often complex: not just the cross-products of numerical domains, but dependently typed objects with complex recursively nested substructures over individually complex types (strings from given sets of strings with complex, consequential interpretations, Boolean values, lists of values, optional values, etc). Constraints on what configuration settings are even functional (don't "break" the system) may not be entirely clear or well documented in forms that can be used easily during optimization procedures. The mathematical characteristics of such optimization problems are often not well understood. Parameters can have non-linear effects on performance. Parameters can be coupled in complex ways through their effects on common performance outputs. One cannot assume in general that performance is a linear or convex function of parameter values. Optimization over discrete spaces of dependently typed objects is not a well understood field, or even one that to our knowledge has been properly formulated before now. The operator might not even have an entirely well defined notion of the objective function, including how to make necessary trade-offs between desirable performance outcomes. One's preferences for trading off increased cost of computing hardware against reductions in the runtime of complex computations might not be adequately appreciated absent experience in the domain. 

%Learning based approaches generally suffer from several common challenges. First, the objective function of a configuration space is unclear due to the complex interactions among parameters. Second, collecting enough and diverse data is not trivial. Some studies demonstrated that users generally just accept the default settings. The training data gathered in such an environment has small variances. For example, a previous work~\cite{ren2013hadoop} found that Hadoop users barely update the settings to gain more performance. Instead, they tend to rely on the default setting and only update it if there is an error in attempted runs. Given such a usage pattern, it is hard to collect training data that are diverse enough to train a good model. The consequence is that a trained model generally has low accuracy in terms of predicting performance close to that in a real operating environment. 

%Other related approaches that we could now evaluate include simulated annealing and random sampling under various distributions. 

% In our work, we recognize the complexity of a configuration space and sample configurations with heuristic algorithms. We show that even with simple sampling strategies, we are able to find configurations that can largely improve system performance.

% Nair et al.~\cite{nair-bad-learners} share our aim to find high-performing configurations for software systems. Their approach is to learn a model to predict the performance of given configurations and to use this model to search for good configurations. The problem they address is that learning an accurate model is computationally infeasible when, as in our work, it is costly to sample the objective function. The insight at the heart of their work is that they don't need to learn a highly accurate model, as long as the model they learn preserves the relative ordering of configurations by performance. Relaxing the constraint of learning an accurate model greatly reduces the cost of learning. They evaluated their approach by testing it on a range of software systems with configuration spaces that are relative small compared to the configuration space of Hadoop that we're considering. 

% Our work differs fundamentally from the work of Nair et al. in that we do not attempt to learn a generalized model -- a function from configuration to performance -- at all. Rather, we employ guided configuration space exploration methods. In this paper we evaluate coordinate descent, a pseudo-gradient descent method, and genetic algorithms. Other related approaches that we could now evaluate include simulated annealing and random sampling under various distributions. 

The fundamental assumption in all of this work is that to find high-performing configurations one needs a generalized predictive model, i.e., a function that can map {\em any} configuration to associated performance with sufficiently good accuracy. How one defines good can vary (e.g., classical accuracy vs. preservation of ordering of configurations with respect to performance~\cite{nair-bad-learners}), but the underlying assumption that one needs to learn such a model remains. 

The intuition that led to the work we report here is that learning {\em generalized} predictive models---that demonstrably produce sufficiently accurate performance estimates {\em for any possible configuration}---is a costly proposition and perhaps one that isn't always necessary. 

\subsection{Alternative Approach}
We propose an alternative idea: that metaheuristic search methods---such as coordinate descent, genetic algorithms, simulated annealing, and so forth---might suffice to find configurations that are much better than baseline defaults, and that this can be done cost effectively without the need to learn generalized performance models. 

In this paper, we claim and present evidence from six experiments involving Hadoop suggesting this is a worthwhile idea to pursue. We exhibit significant performance benefits obtained at costs that are by any measure reasonable (in time and money). We do not try to present a head-to-head comparison of this method against approaches that are based on learning generalized models. Such a comparative evaluation is left to future work.

As with learning-based approaches, our meta-heuristic search approach also requires dynamic evaluation of the performance objective function, so we, too, are concerned with reducing the cost of such sampling. Our second main insight is that rather than reducing the {\em number} of evaluations of the objective function, we can reduce the {\em cost of each call} by evaluating the objective function using only small input problem instances, in hopes that the ``good'' configurations we find for small problem instances will also perform well on problem inputs orders of magnitude larger. The second main contribution of this work is experimental tests and data that support this {\em scale-up hypothesis}. 

\subsection{Case Study}
In this paper, we take Hadoop as a case study. Hadoop and its variants are widely used in major data-and-computation-intensive industrial and busines processes. Finding ways to reduce the cost of big-data Hadoop computations would have significant impacts for enterprises in many sectors of the economy. 
Hadoop also clearly has a complex and performance-critical configuration space. It has more than nine hundred configuration parameters distributed across its core file system (HDFS), map reduce, and cluster management (Yarn) subsystems. Some parameters serve to enable or disable certain functions. Others adjust everything from file names to resources allocation policies to algorithmic strategies: e.g., scheduling strategies, how to split up input data, whether to compress outputs, etc. 

Furthermore, research in the Hadoop community~\cite{ren2013hadoop} has shown that users rarely and barely change default configuration parameters, and usually only to correct misconfiguration errors. They offer two explanations. First, default configurations might be viewed as good enough. Second, the configurations are complex and hard enough to understand that users aren't comfortable changing them.

In this paper, we focus on configuration parameters that affect system runtime performance. Some, e.g., file names, probably do not. We used our own domain knowledge to select the more than one hundred potentially performance-related configuration parameters. We are thus working a vast configuration space and in a setting in which evaluating the actual objective function requires very expensive actual runs of Hadoop, each of which, including set-up, takes at a minimum several minutes.

\subsection{Summary of Results}
We present data from six experiments using Hadoop to solve three kinds of problems from the HiBench~\cite{huang2010hibench} suite (sort, wordcount, and terasort), using two metaheuristic search methods (coordinate descent and genetic algorithms). Our algorithms found configurations that improve performance by amounts ranging from 6.5\% to 56.7\%, with configurations found using small instances sometimes providing even greater improvements as input size is scaled by factors of 10X and 100X. We details these results in Section~\ref{sect:results}.


%Our hypothesis at the heart of our work is that at least in some important cases, we can radically reduce the cost of such a search by using only small inputs to sample the objective function, in hopes that the resulting configurations will provide greatly improved performance even for inputs orders of magnitude large.
%In this paper we present experimental data that at least some important cases appear to support this hypothesis. 
%We explored Hadoop's configuration space using three small problem instances in an attempt to find better configurations. We then tested experimentally the hypothesis that these configurations improve performance relative to default configurations even when used for jobs \textit{10x} and \textit{100x} bigger.

%Our experimental results show the resulting configurations of genetic algorithm can produce even larger performance improvement for larger job instances than small ones. 

% We analyze the effectiveness of cyclic coordinate descent and genetic algorithm in exploring configuration space of software systems, the cost of doing that, and insights in found configurations. We also talk about limitations of this work, threats to the validity, and future research.

% \noindent
% \textbf{Scale-Out Hypothesis: Configurations found with representative jobs can produce similar performance for other similar jobs.}
% Running our approach for each single job could reduce its usability due to the cost to explore configurations. In this hypothesis, we test whether explored results with representative jobs could be applied to other similar jobs.

\subsection{Structure of Paper}
The rest of this paper is organized as follows. Section~\ref{sect:approach} presents our technical approach. Section~\ref{sect:experiment} discuss the experiment design and Section~\ref{sect:results} presents results of a case study on Hadoop system. Section~\ref{sect:interpretation} interprets our results and answer research questions. Section~\ref{sect:evaluation} discusses strengths, limitations, and significance of this work. Section~\ref{sect:related} reviews previous related work. At last, section~\ref{sect:conclusion} concludes this paper.


==> intro_back.tex <==
\section{Introduction}
\label{sect:introduction}

Many software systems are highly configurable and can be tailored to different needs and environments. In practice, however, people  find it hard to exploit  configurability. Instead, they simply use prepackaged, or \textit{default}, configurations~\cite{ren2013hadoop}. As a result, they often leave significant performance potential unrealized. Configuring for performance is important~\cite{xu2015hey}, and
especially so for big data systems because~\enquote{even a small performance improvement translate into significant cost savings due to the scale of computations involved~\cite{jia2016auto}}.

Finding high-performing (or \textit{good}) configurations for big data systems is hard. Their configuration spaces are vast, and their configuration-to-performance mapping functions, complex. They have multiple configurable sub-systems~\cite{white2012hadoop}. Hadoop, for example, has about 900 parameters across 4 sub-systems. Some parameters, e.g., numeric ones, have many values. Parameters also have diverse types, including optional and dependent substructures.  For example, setting one Boolean parameter to {\em true} can enable a feature, requiring values for all of its parameters. Parameters can also be constrained by external values. 
For example, in a multi-core system, one cannot set the  \textit{number-of-core} value to a number larger than the number of available cores.  Configuration-to-performance functions are not well understood: e.g., how parameter values interact. Also, due to its discrete nature, typical mathematical optimization methods do not apply~\cite{louviere2011design}. Finding good configurations ends up as a black-art~\cite{Joshi:2012:AHP:2188286.2188323}.

%such spaces involve thousands of values for each of the dozens or hundreds of parameters, and many constraints on how values can be set. Moreover, configurations are often not just numerical vectors, but can have fields with diverse types, as well as optional and dependent substructures. For example, setting one Boolean parameter to {\em true} can enable an entire subsystem, requiring many more configuration values. Similarly, these spaces can also be parameterized by external values: e.g., one cannot set a Hadoop \textit{number-of-CPUs} parameter to a number larger than the available number of CPUs. Analysts often don't know key properties of configuration-to-performance functions: e.g., how parameters interact, whether properties analogous to convexity, linearity, and differentiability, apply, etc. 
%For such complex and discrete problems, standard mathematical optimization methods is known not to apply well~\cite{}.  

For traditional systems, the problem of finding better configuration  has given rise to a significant body of work. %~\cite{siegmund2012predictperf, siegmund2015performance, zhang2015performance, venkataraman2016ernest,sarkar2015cost,guo2013variability}. 
In general, these techniques involve the following steps: 
(i) deploy different sampling strategies to select a set of valid and representative configurations~\cite{gogate2006new,chakraborty2014distribution,lei2008ipog,johansen2012algorithm,marijan2013practical,kaltenecker2019distance},
(ii) use the sampled configurations to dynamically profile %by running
the system under test,
(iii) use Machine Learning (ML) models to learn the configuration-to-performance mapping functions from the collected traces~\cite{siegmund2012predictperf,siegmund2015performance,guo2013variability,nair-bad-learners,nair2018finding}, and finally, 
(iv) use the learned models to find good configurations.
Success of such learning-based approaches depends heavily on the size and the quality of the sampled configuration set used for training. 
It turns out for complex, configurable systems, such as ours, the measurement data  often do not generalize well~\cite{nair-bad-learners}. 
In response, Nier \etal proposed a rank-based learning approach. Instead of trying to learn models for predicting absolute performance, they learn models that just predict whether one given configuration is better than another. They showed such predictors can be learned with significantly fewer {\em samples} than residual-based approaches  %(their target is to minimize something like mean squared error) 
and is still useful.

%They are  based on dynamic profiling of running systems to learn models to predict configuration-to-performance objective functions and then using these models to help find good configurations. 
However, for big-data systems, these existing techniques struggle to scale, especially due to following two reasons:

\noindent
(1) {\em Cost of collecting training data.} The cost is prohibitively large~\cite{weiss2008maximizing} in big-data systems. 
For example, in a typical Hadoop system, a single run of a simple sorting task for a typical workload (data size=3.2GB) can take up to 14 minutes.
Thus, it would be hard to amortize the initial cost of collecting enough traces to train a model. 
Suppose, for example, that it takes one thousand runs of a production-scale big data job---perhaps one that runs once a day---to find a configuration that yields a ten percent performance improvement. It would then take ten thousand production runs, or more than twenty-five years, to break even. Multiple orders of magnitude of cost reduction would be needed for such a method to be practical.


% The need to radically reduce search costs, if benefits net of costs are to be obtained, is clear. Suppose, for example, that it takes one thousand runs of a production-scale big data job---perhaps one that runs once a day---to find a configuration that yields a ten percent performance improvement. It would then take ten thousand production runs, or more than twenty-five years, to break even. Multiple orders of magnitude of cost reduction would be needed for such a method to be practical.

\noindent
(2) {\em Complex Configuration Space.}
The configuration-finding problem for big data systems involves significantly larger number of dimensions than addressed in most previous work. For these systems it is hard to learn even rank-preserving models with high accuracy (see in~\Cref{sect:results}).  One might try Neural Networks (NNs)~\cite{ha2019DeepPerf}. However, NNs require large amounts of data for training, and the cost of even collecting such data for big-data systems would be prohibitively high~\cite{pavlo2009comparison}.

% Much of it is based on dynamic profiling of running systems to learn models to predict configuration-to-performance objective functions and then using these models to help find good configurations. The cost of doing this for big data systems is high~\cite{weiss2008maximizing} and hard to amortize. Measurement data also often do not generalize well for such complex, configurable systems~\cite{nair-bad-learners}. 


% to achieve the desired goal. 

% The configuration-finding problem for big data systems involves much higher-dimensional spaces than addressed in most previous work. For these systems it is hard to learn even rank-preserving models with high accuracy (see in~\Cref{sect:results}).  One might try Neural Networks (NNs). However, NNs require large amounts of data for training, and the cost of such data for big-data systems would be very high~\cite{pavlo2009comparison}.

% (i) The parameter space is huge (ii) each sample takes time to get
% (iii) Similar patterns tend to have similar sub-problems....

%\begin{itemize}
%    \item 
%    Find a {\em good enough} configuration within a limited computation budget to achieve better performance. 
%    %that can achieve better performance \wrt the others.
%    %thus the challenge is to learn \textit{good enough} models with as few samples as possible. 
%    \item
%    Find the configuration with {\em as little cost as possible}.
%\end{itemize}

Thus, given the cost of collecting data in a big data system and the number of samples needed to train a good model, the popular learning based approaches may not be feasible or even necessary (see in~\Cref{sect:results}) in this setting. 
Instead, we can aim for finding a \textit{near optimal} configuration\textemdash which performs better than all other known configurations, within a given budget using guided sampling.
A meta-heuristic optimization strategy that can pick {\em diverse} configurations with {\em high discriminatory power} can realize this goal.
In this paper we present results for such an approach based on Evolutionary Markov Chain Monte Carlo (EMCMC) methods, in particular.
A nice property of EMCMC is that it tries to estimate the target distribution, \ie draws more samples from important regions and yet maintains some sample diversity; Thus, it avoids quick convergence to local optima. 

% Our key insight is that learning predictive models that are accurate over the entire configuration spaces may not be necessary if one's aim is just to find \textit{good enough} configurations within limited budget---that performs better than other known configurations. 
% To achieve this aim in our setting, \ie limited budget to explore a complex high-dimensional space, we may not need a learning-based  prediction model.
% Instead, a meta-heuristic optimization strategy that can pick {\em diverse} configurations with {\em high discriminatory power} can be sufficient to achieve a near-optimal performance. 
% In this paper we present results for such an approach based on Evolutionary Markov Chain Monte Carlo (EMCMC) methods, in particular.


To further reduce the cost of collecting the samples, in particular the dynamic traces, we devised, implemented, and evaluated two ideas. First, we hypothesized that big data jobs %one hundred times 
running with inputs significantly smaller than those used in production can be used as proxies for sampling configuration-to-performance objective functions and that improvements found using these smaller jobs would still hold for much larger ones. We call this our {\em scale-up} hypothesis. Second, we hypothesized that better configurations for one kind of job would yield improvements for \textit{dynamically similar} jobs, entirely avoiding the need for redundant sampling and thus, it will amortize the cost of profiling over many similar jobs. We call this as our {\em scale-out} hypothesis. 

We conducted experiments using the Hadoop and Spark frameworks, and five canonical big data problems defined by the HiBench~\cite{huang2010hibench} benchmark suite. For each problem, HiBench provides a broad range of job sizes. We measured improvements by comparing CPU time under default (experimental control) configurations with (treatment) configurations found using (a) our approach, and (b) competing alternatives. Our approach results showed performance gains from 14.2\% to 25.2\%.  Our approach also outperformed a same-cost {\em random} search by 17\% to 125\%, and the model-learning approach of Nair et al. by 5\% to 1700\%.
%is far less effective as it only improves jobs' performance from 1.4\% to 20.4\%, in which most cases are far behind our approach. We will discuss the detailed findings in RQ4 and RQ5.

%The main contribution of this paper, then, is the experimental demonstration that an EMCMC approach to configuration optimization combined with sampling cost reduction and avoidance techniques can cost-effectively produce major improvements in runtime performance, thus financial costs, of important classes of big data computations.

These improvements, combined with an assumed 100X reduction in sampling costs based on our scale-up strategy, suggest that our approach could produce break-even benefits for large, daily big data jobs in just a few months. Furthermore, our results suggest that results from one task could immediately benefit similar jobs. Our conclusion then, and the main contribution of this work, is the idea, supported by experimental evidence, that the combination of an evolutionary Markov Chain Monte Carlo sampling with scale-up and scale-out cost-reduction methods has strongly demonstrated potential to produce industrially important performance benefits to users of big data systems.

%The main contribution of this paper includes:
%
%\begin{itemize}[leftmargin=*]
%    \item 
%    We present a novel approach to searching high-dimensional configuration space for big-data system to achieve better performance. %high-performing configurations.
%    The search performance outperforms the base-line system with significant margin. 
%    \item 
%    Scale-up hypothesis results show that configurations found with small job instances also work for larger jobs, thus saving significant experimental cost.
%    \item 
%    Scale-out hypothesis results show that configurations found with representative jobs can also improve the performance of similar %jobs, thus saving significant experimental cost.
%\end{itemize}


%The rest of this paper is organized as follows. Section~\ref{sect:background} presents background information on configuration spaces and EMCMC algorithms. Section~\ref{sect:approach} presents our approach. Section~\ref{sect:experiment} discuss our experimental design for evaluating our approach. 
%Section~\ref{sect:rq} talks about our research questions. Section~\ref{sect:results} presents our experimental results. Section~\ref{sect:related} compares and contrasts our approach with previous related work. Section~\ref{sect:threats} discusses limitations of our approach, future work, the threats to the validity of our conclusions. Section~\ref{sect:conclusion} concludes.



%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
% commented out
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}


\subsection{Case Study}
In this paper, we take Hadoop as a case study. Hadoop and its variants are widely used in major data-and-computation-intensive industrial and business processes. Finding ways to reduce the cost of big-data Hadoop computations would have significant impacts for enterprises in many sectors of the economy. 
Hadoop also clearly has a complex and performance-critical configuration space. It has more than nine hundred configuration parameters distributed across its core file system (HDFS), map reduce, and cluster management (Yarn) subsystems. Some parameters serve to enable or disable certain functions. Others adjust everything from file names to resources allocation policies to algorithmic strategies: e.g., scheduling strategies, how to split up input data, whether to compress outputs, etc. 

Furthermore, research in the Hadoop community~\cite{ren2013hadoop} has shown that users rarely and barely change default configuration parameters, and usually only to correct misconfiguration errors. They offer two explanations. First, default configurations might be viewed as good enough. Second, the configurations are complex and hard enough to understand that users aren't comfortable changing them.

In this paper, we focus on configuration parameters that affect system runtime performance. Some, e.g., file names, probably do not. We used our own domain knowledge to select the more than one hundred potentially performance-related configuration parameters. We are thus working a vast configuration space and in a setting in which evaluating the actual objective function requires very expensive actual runs of Hadoop, each of which, including set-up, takes at a minimum several minutes.

\end{comment}

==> phase1.tex <==
\subsection*{Phase-\rom{1}: Pre-processing the configuration space}  

A typical configuration space for big-data framework is high dimensional and complex. 
For instance, total number of parameters for Hadoop and Spark are 901 and 212 respectively (see Table~\ref{tab:subj}). Further, these parameters can have data types ranging from boolean, integer, float, string, and categorical. Thus, the configuration space forms by varying the total number of potential combinations can be exponentially  large (\eg if n parameters can each takes m values, the configuration space can grow upto $m^n$). 
Moreover, some of the parameters interact with others. 
For example, in Hadoop, parameters block size and minimum data split size together decide 
in how many fragments the input data will be divided into~\footnote{https://wiki.apache.org/hadoop/HowManyMapsAndReduces}.
Similarly, the number of CPU cores of the resource manager and map/reduce tasks constrain each other, as the total numbers cannot be larger than the number of physical cores. Such diverse data-types and inter-parameter interactions increase the complexity of big-data configuration space significantly. 


Thus, we first reduce the dimension of the configuration space of a framework. This involves two steps: (i) choose important features, (ii) among the important features, study only critical range of values. 
To select the important features, we use our domain knowledge to remove parameters unrelated to our objective function, \ie performance in this case. 
We first filter out the parameters that may not have any influence on a job's performance, at least not directly. 
This part is manual. The first author went through the parameter descriptions by studying their manual and previous literature~\chong{cite} and filtered out the irrelevant parameters. The manual studu took a week for one research. How to automate such feature selection is itself very interesting and will be part of our future work. 

We remove five main classes of parameters for Hadoop: 
(i) version related, \eg, \emph{java.runtime.version} and \emph{java.class.version}.%  values are strings like ``1.8.0''. 
These parameters describe the current system configuration (\eg Java version ``1.8.0") but have no impact on the CPU time given a cluster. 
(ii) path-related, \eg, \emph{hadoop.bin.path} and \emph{hadoop.log.dir}. Such parameters do not strongly influence computation or CPU time. 
(iii) authentication related, \eg, \emph{hadoop.login} and \emph{hadoop.http.authentication.kerberos.keytab}. 
(iv)  server-address related, \eg, \emph{mapreduce.jobtracker.http.address}, these parameters are similar to those log directory related parameters. 
The last class are (v) ID/name related, \eg, \emph{mapreduce.output.basename}, because jobs names do not impact their performance. 
Thus, we reduced the number of parameters from $901$ to $44$. %Details are in our Github repository.

For Spark, there are 212 total parameters in this version. They are listed in multiple categories on Spark's website\footnote{https://spark.apache.org/docs/2.2.0/configuration.html} with detailed explanation. 
Here we selected parameters that are related to runtime performance. Specifically, we selected 27 parameters from \textit{Runtime Environment}, \textit{Shuffle Behavior}, \textit{Compression and Serialization}, \textit{Memory Management}, and \textit{Execution Behavior}, and \textit{Scheduling} categories.

We further discretize the configuration space by defining sampling values for each parameter, varying by parameter type. Boolean parameters are sampled for only true and false values. We sample numerical parameters at a few values less and greater than their defaults. For string-valued parameters (\eg, as Java virtual machine settings) we provide lists of alternative values. 


==> related_back.tex <==
%!Tex root=icse18.tex

\section{Related Work}
\label{sect:related}
It's difficult to understand how complex configurations impact system performance. Some previous works tried to build performance prediction model for configurable systems to understand configuration-to-performance relationship. Siegmund et al.~\cite{siegmund2015performance} proposed an approach to learn the influences of individual parameters on system performance and possible interactions among them. They assume that most common case is two-way interactions happen between binary and numeric options. In order to uncover such information with learning based approach, they used different sampling strategies to generate learning sets. 
%They first sample values for binary options with heuristic sampling and then for numeric options with different sampling strategies. 
In the learning model, they added interaction terms for binary and numeric option combinations. This approach combines domain knowledge (interactions among parameters) in the sampling strategies to generate effective training data. The evaluations results on several systems showed that this approach can achieve relative high accuracy compare to previous work. But still, the average error rate is 19\% and some models have that as high as 37.4\%. We recognize the complexity of a configuration space and sampled configurations with an interaction-free strategy and genetic algorithms assuming full-way interactions. We show that even with simple sampling strategies, we are able to find configurations that can largely improve system performance. In this work, we didn't explicitly consider the semantic meaning of all parameters and constraints in a configuration space. However, our approach is able to integrate such information implicitly. In our implementation, if a configuration breaks the system or triggers any unexpected error, the algorithm returns the maximum integer value the machine can represent to mark the configuration as a wrong configuration. 

Nair et al.~\cite{nair-bad-learners} share our aim to find high-performing configurations for software systems. Their approach is to learn a model to predict the performance of given configurations and to use this model to search for good configurations. The problem they address is that learning an accurate model is computationally infeasible when, as in our work, it is costly to sample the objective function. The insight at the heart of their work is that they don't need to learn a highly accurate model, as long as the model they learn preserves the relative ordering of configurations by performance. Relaxing the constraint of learning an accurate model greatly reduces the cost of learning. They evaluated their approach by testing it on a range of software systems with configuration spaces that are relative small compared to the configuration space of Hadoop that we're considering. Our work differs fundamentally from theirs in that we do not attempt to learn a generalized model -- a function from configuration to performance -- at all, but employing guided configuration space search algorithms.

In some previous work~\cite{Siegmund:2012:performance,guo2013variability,apel2013feature}, several automatic ways are presented to detect performance-related feature interactions to improve the accuracy of a prediction model. Meinicke et al.~\cite{meinicke2016complexity} studied the complexity of configuration spaces of some open-source software systems by running multiple configurations at the same time and compare the differences in control and data flow. They found that the complexity degrees of most configuration spaces of the studied Java programs is not as much high as configuration space indicates, but still state-of-the-art strategies cannot handle such large space. In this project, we leveraged domain knowledge to select parameters that could influence the performance of a given system. We also treat a system as a black-box and analyzed parameters' impact on performance with dynamic benchmark. For Hadoop system, a large number of options have been thoroughly studied by some other work and summarized in~\cite{Bonifacio:research_review}, which gives us enough information to determine which ones are performance related.

Zhang et al.~\cite{zhang2015performance} assumes all options are independent and can be converted to boolean variables. They thus formulated the problem of performance prediction as learning the Fourier coefficients of a function. This approach can learn a performance model fast. However, in practice, not all parameters are boolean and converting arbitrary variables to boolean could dramatically increase the feature space. Venkataraman et al.~\cite{venkataraman2016ernest} built a performance prediction framework for shared cloud computing infrastructure. The insight is that the behaviors of a job can be predicted. They derived the performance model by running a given job with a set of small samples. The main purpose of their work is to propose suitable resource allocation for a given job, where we implicitly consider broader factors, like interactions among parameters. All these learning based approaches suffer from the problem of lacking of high quality training data. Users tend to use the default setting~\cite{ren2013hadoop} in practice and only tune it when errors happened. Such usage pattern creates historic traces that cover a small area in a configuration space. Therefore, a performance prediction model trained using such data is usually inaccurate. 

% meta-heuristic search configuration spaces
In other research fields, many works have proved that meta-heuristic search can find alternative systems with better performance. 
Baltz et al.~\cite{baltz2017nuclearfusion} presented an exploring algorithm called Optometrist which includes human in finding good configurations for complex engineering systems. They applied this algorithm in a plasma fusion system to stochastically sample configurations that can reduce the energy loss rate and increase the plasma temperature. In such a system, thousands of parameters exist and many of them interact among others and with external parameters, there are multiple objective metrics need to be optimized and the safety constraints are not well defined. In order to reduce the cost of finding good configurations, they introduce the concept of meta-parameters to group parameters so that no interactions exist among these groups. The algorithm only needs to explore multiple small spaces rather than a huge one, which dramatically speedup the learning and optimization procedure. Introducing human in the loop leverages the domain knowledge to make decisions for metrics that cannot be well computed by machine. Their work is highly related to ours as we all work in optimizing the configurations of complex and high dimension engineering systems. They reduce the cost by introducing the concept of meta-parameters, whereas we achieve that by guiding the exploring procedure with small and low-cost jobs.
In the embedded hardware design domain, Palermo et al.~\cite{palermo2005multi} uses heuristic algorithms to find configurations from an architectural design space to compute an approximation of Pareto frontier with respect to energy and delay trade-offs. In software systems, such frontier is hard to compute because there are many optimization figures, like CPU time, memory, reliable and so on. Zhang et al.~\cite{zhang2004self} used heuristic algorithms to find better settings for single-level configurable cache to avoid power-consuming cache flushing, where they optimized four cache parameters including one boolean parameter and three numerical parameters. The space they worked on is much smaller and simpler than even a tiny size software system. In robotic motion planning domain, Jaillet et al.~\cite{jaillet2010sampling} used stochastic sampling to find globally low-cost paths for robotics with an arbitrary user given cost functions. Burns et al.~\cite{burns2005toward} used heuristic sampling to solve the connectivity problem in robotic motion planing field. These works solved similar problems with ours in other engineering fields. The common challenge is that given the vast size and complex structure of configuration spaces, it's hard to find a good configuration. Meta-heuristic search algorithms seem promising to reveal high-value solutions.

In the software engineering field, recently, many works have shown that heuristic search algorithms can be leveraged to solve various problems.
%Harman~\cite{harman-search-future} reviewed the application of search and optimize technique in eight software engineering domains, as well as the open problems and challenges.
Weimer et al.~\cite{weimer-genetic-repaire} used genetic algorithm to find correct candidate code snippets to repair buggy code. Jia and Harman~\cite{jia-higherorder-test} used automated search-based techniques to find rare but valuable test cases. McMinn~\cite{MacMinn-test-generation} surveyed the application of search techniques for automated test data generation. In this project, we utilize heuristic search algorithms to discover high-value configuration settings. There are many works in applying heuristic algorithms in search-based software engineering and getting promising results. Weimer et al.~\cite{weimer-icse2012} reported that they can fix bugs with only \$8 each, where they used genetic programming to mutate code statements to create a large space of new variants and then try to fix the buggy code by replacing it with new code variants randomly sampled from the generated space. Le~\cite{le2015-compiler-mcmc} used Markov Chain Monte Carlo (MCMC) techniques to generate program variants with different control- and data-flow. They then used these diverse programs to uncover deep bugs in compilers. They successfully found some bugs in popular compilers like GCC and LLVM. Whittaker and Thomason~\cite{whittaker1994markov} presented an approach to statistically test software against failures. They used a Markov Chain model to generate test inputs, and thus to study under what usage cases a software could fail. At the very beginning, we also considered MCMC as a candidate algorithm. However, we found out that the distribution of performance with respect to configurations is not well defined and it's hard to find a probability distribution to estimate. While most previous works focused on system correctness, this project focuses on system performance optimization problem. We use cyclic coordinate descent and genetic algorithm to sample system settings from a configuration space to improve system performance.



==> rq_back.tex <==
\subsection{Research Questions}
\label{sect:rq}
\label{sect:hypothesis}

%In this section, we discuss three key research questions underpinning this work. 
% However, due to the big-data nature of data processing infrastructures, the exploration cost could be too high for an organization to afford. Therefore, we propose this multi-resolution approach to first explore the whole configuration space with small job instance. Once we found some good configurations, we evaluate them with larger (10X and 100X) job instances to further pick out better configurations. Using small job instance to explore the whole configuration space can save a large amount of cost, but it could lead to some \textit{not-so-good} configurations. This multi-resolution can avoid such glitches by adding post-processing steps to the exploration phase.
\noindent
We will now discuss four research questions underpinning this work.  

\RQ{1}{\rqa}

We investigate this RQ \wrt small workloads only. The question is can we find better configurations for small jobs using small inputs in sampling. \tool runs the benchmark jobs by setting the workload size  ``Small'' in the HiBench configuration file. HiBench generates a detailed report after each run, with diverse performance information including CPU time. For our experiments, small inputs are more than three hundred megabytes for ``micro'' jobs. Each execution in HiBench contains two steps: data preparation and job execution. However, we manually prepare the data so that each job under test can be run with the same workload. Hence, we modify HiBench to bypass its first step and run jobs with only user-provided data. At the end of each exploration, some good configurations are output along with their performance data, as well as how they compared to the baseline configuration. We then evaluate the validity of the first RQ by assessing {\em whether we gain significant speedups for small jobs}.
% The data preparation step for jobs in the \textit{Micro Benchmark} category have only \textit{Map} tasks and no \textit{Reduce} task. To evaluate how a configuration performs in the common scenario, where jobs contain both \textit{Map} and \textit{Reduce} tasks, we instrument HiBench so that in one set of experiments, the job preparation step only run once at the beginning of the whole set of experiments.
% By doing this, we make sure that all jobs using the same dataset.

\RQ{2}{\rqb}

While using small workloads during exploration can save significant cost, a high performing configuration found with smaller workload may not work well for larger workloads. To investigate RQ2, after finding improved configurations using small inputs, we run the same HiBench job as used during exploration with ``Large'' and ``Huge'' inputs, 10X and 100X times larger than those used in exploration (thus more than 3-gigabyte and 30-GB inputs). We profile both the default and discovered configurations, choosing the top 50 configurations found in RQ1 for each job. We record the CPU times of each execution running with the ``Large'' and ``Huge''  workloads. We evaluate the {\em scale-up} hypothesis by checking for  significant gains in performance when we scale up input sizes by up to two orders of magnitude.

\RQ{3}{\rqc}

The scale-out hypothesis suggests that a good configuration found for one kind of job, A (e.g., Word Count), will also produce performance gains for a similar kind of job, B (e.g., Sort). If this hypothesis holds true, we could further reduce exploration costs by applying a configuration found for one kind of job to other similar jobs without repeating a costly exploration process. As detailed further below, we test this hypothesis by evaluating performance gains for job B using configurations found for job A.

\RQ{4}{\rqd}

After investigating the effectiveness of EMCMC in finding high-performing configurations, we study how it performs comparing to more straightforward sampling strategies. Here we compare EMCMC with a purely random sampling strategy. A pure random approach samples a value for a parameter in the uniform distribution, which means each value in the value range has the same probability to be selected. To compare with EMCMC, we run the pure random sampling strategy to generate the same number of configurations and profile their performance with small data sets. We also conduct the scale-out validation to verify how found good configurations perform under larger input data sets. At last, we compare EMCMC and pure random sampling strategy regarding how they perform in finding high-performing configurations in ''Huge`` data sets.

\RQ{5}{\rqe}
Many previous work solves the problem of finding high-performing configurations with learning-based approaches. In this line of work, researchers first gather system usage data to train a prediction model, and then use this model to find good configurations. While most work tries to build high-accuracy models, Nair et al.~\cite{nair-bad-learners} argue that a model that can preserve configuration ranking is enough to find good configurations. They compared their rank-based models with residual-based models and demonstrated that a rank-based model has the same or higher effectiveness in finding high-performing configurations.

In this work, we compare our approach that based on meta-heuristics search algorithms with the work of Nair et al., to find out which approach is more effective in finding high-performing configurations. We adopt the same criterion used in their paper: the rank-difference of configurations.

%====

%Our method is based on intelligently sampling  configurations and measuring performance. Such sampling can incur huge overhead, especially for big-data jobs\textemdash. The cost  may be too high for an organization to afford. We propose what amounts to a kind of multi-resolution approach, wherein we use small jobs for sampling while validating the results against target jobs at much greater scale. This reduces the cost of search by orders of magnitude.  First, we explore the configuration space with small workload. Once some better configurations are found, we perform a {\em scale-up} test by  checking whether larger (10X and 100X) workloads also benefit(RQ2). 
%Even if we are successful with our scale-up hypothesis testing, 
% % finding an optimal configuration for each big-data job can still be expensive, especially for organizations that often run different jobs. Also, it might be difficult to change the configuration of the clusters each time when a new job. This leads to {\em scale-out} experiment:  we check whether optimal configurations found from one job can be effective for the similar type of other jobs (RQ3).


% Thus, we begin with asking: 

%====
%The results show that four out of five Hadoop jobs are similar. They are WordCount, Sort, Terasort, and PageRank. NutchIndex is not similar to them. For Spark jobs, WordCount, Sort, TeraSort, RF, SVD are highly similar. Other jobs have low similarities.

% \begin{itemize}
%     \item \textbf{H1:} Our approach can find significantly better configurations than the baseline configuration.
%     \item \textbf{H2:} The configurations found with small data inputs work well for larger inputs.
%     \item \textbf{H3:} The configurations found with a representative job work well for other similar jobs.  
% \end{itemize}

%\subsubsection{H1: Approach effectiveness}
%\subsubsection{H2: Scale-up hypothesis} 
%\subsubsection{H3: Scale-out hypothesis}



==> tables/hadoop_performance.tex <==















% \begin{table*}[!thpb]
% 	\scriptsize
% 	\setlength{\tabcolsep}{0.4cm}
% 	\centering
% 	\caption{{Performance improvement for Hadoop jobs from three sampling strategies}}
% 	\label{tab:hadoop-perf-improvement}
% 	\begin{tabular}{l|c|c|c|c|c|c|c|c|c}
% 		\hline
% 		& \multicolumn{3}{c|}{\textbf{EMCMC}} & \multicolumn{3}{c|}{\textbf{Genetic Algorithm}} & \multicolumn{3}{c}{\textbf{Random Sampling}} \\ \hline
% 		& \textbf{Exploration} & \multicolumn{2}{c|}{\textbf{Scale-up}} 
% 		& \textbf{Exploration} & \multicolumn{2}{c|}{\textbf{Scale-up}} 
% 		& \textbf{Exploration} & \multicolumn{2}{c}{\textbf{Scale-up}} \\
% 		%& \textbf{Phase} & \multicolumn{2}{c|}{\textbf{Phase}} & \textbf{In Exploration} & \textbf{Phase} & \multicolumn{2}{c|}{\textbf{Phase}} & \textbf{Phase} & \multicolumn{2}{c}{\textbf{Phase}}\\
% 		\hline
% 		\textbf{Job}               & \textbf{Small} & \textbf{Large} & \textbf{Huge} & \textbf{Small} & \textbf{Large} & \textbf{Huge} & \textbf{Small} & \textbf{Large} & \textbf{Huge} \\ \hline
% 		\textbf{WordCount}         
% 		    & 12.5\%         & 15.6\%         & 21.5\%        
% 		    & 6.5\%          & 9.8\%          & 11.6\%        
% 		    & 5.6\%          & 9.7\%          & 14.6\%        \\
% 		\textbf{Sort}              
% 		    & 72.1\%         & 7.7\%          & 15.8\%        
% 		    & 70.6\%         & 11.4\%         & 10.3\%        
% 		    & 60.6\%         & 5.3\%          & 13.5\%        \\
% 		\textbf{TeraSort}          
% 		    & 27.4\%         & 16.1\%         & 18.3\%        
% 		    & 21.6\%         & 17.2\%         & 15.9\%        
% 		    & 11.6\%         & 8.6\%          & 11.1\%        \\
% 		\textbf{PageRank}          
% 		    & 32.7\%         & 44.7\%         & 25.2\%        
% 		    & 46.4\%         & 17.5\%         & 21.2\%   
% 		    & 32.9\%         & 12.0\%         & 11.2\%        \\
%  		\textbf{NutchIndex}        
%  		    & 7.1\%          & 18.7\%         & 14.2\%        
%  		    & 5.7\%          & 11.5\%         & 13.4\%        
%  		    & 10.4\%          & 14.4\%         & 12.0\%        \\ 
%  		%\hline
% % 		\textbf{\textit{*Average}} & 30.4\%         & 20.6\%         & 19.0\%        & 30.2\%         & 13.5\%         & 14.5\%        & 24.2\%        & 10.1\%         & 13.1\%        \\
% 		\hline
% 	\end{tabular}
% 	\vspace{-.5cm}
% \end{table*}




% \begin{table*}[!thpb]
% 	\scriptsize
% 	\setlength{\tabcolsep}{0.4cm}
% 	\centering
% 	\caption{{Performance improvement for Hadoop jobs from three sampling strategies}}
% 	\label{tab:hadoop-perf-improvement}
% 	\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c}
% 		\hline
% 		& \multicolumn{4}{c|}{\textbf{EMCMC}} & \multicolumn{3}{c|}{\textbf{Genetic Algorithm}} & \multicolumn{3}{c}{\textbf{Random Sampling}} \\ \hline
% 		& \textbf{Exploration} & \multicolumn{2}{c|}{\textbf{Scale-up}} & \textbf{Best Conf.} & \textbf{Exploration} & \multicolumn{2}{c|}{\textbf{Scale-up}} & \textbf{Expl.} & \multicolumn{2}{c}{\textbf{Scale-up}} \\
% 		& \textbf{Phase} & \multicolumn{2}{c|}{\textbf{Phase}} & \textbf{In Exploration} & \textbf{Phase} & \multicolumn{2}{c|}{\textbf{Phase}} & \textbf{Phase} & \multicolumn{2}{c}{\textbf{Phase}}\\
% 		\hline
% 		\textbf{Job}               & \textbf{Small} & \textbf{Large} & \textbf{Huge} & \textbf{Small} & \textbf{Large} & \textbf{Huge} & \textbf{Small} & \textbf{Large} & \textbf{Huge} \\ \hline
% 		\textbf{WordCount}         & 12.5\%         & 15.6\%         & 21.5\%        & 20.1\% & 6.5\%          & 9.8\%          & 11.6\%        & 5.6\%          & 9.7\%          & 14.6\%        \\
% 		\textbf{Sort}              & 72.1\%         & 7.7\%          & 15.8\%        & 15.7\% & 70.6\%         & 11.4\%         & 10.3\%        & 60.6\%         & 5.3\%          & 13.5\%        \\
% 		\textbf{TeraSort}          & 27.4\%         & 16.1\%         & 18.3\%        & 14.5\% & 21.6\%         & 17.2\%         & 15.9\%        & 11.6\%         & 8.6\%          & 11.1\%        \\
% 		\textbf{PageRank}          & 32.7\%         & 44.7\%         & 25.2\%        & 22.9\% & 46.4\%         & 17.5\%         & 21.2\%        & 32.9\%         & 12.0\%         & 11.2\%        \\
%  		\textbf{NutchIndex}        & 7.1\%          & 18.7\%         & 14.2\%        & 11.2\% & 5.7\%          & 11.5\%         & 13.4\%        & 10.4\%          & 14.4\%         & 12.0\%        \\ 
%  		%\hline
% % 		\textbf{\textit{*Average}} & 30.4\%         & 20.6\%         & 19.0\%        & 30.2\%         & 13.5\%         & 14.5\%        & 24.2\%        & 10.1\%         & 13.1\%        \\
% 		\hline
% 	\end{tabular}
% 	\vspace{-.5cm}
% \end{table*}

==> tables/scale-out.tex <==



==> tables/spark_performance.tex <==
\begin{table}[h]
\scriptsize
	\centering
	\caption{{Performance Improvement of \tool for Spark jobs}}
	\label{tab:spark-perf-improvement}
	\begin{tabular}{l|P{2cm}|P{2cm}}
		\hline
		\textbf{Job}        & \textbf{Exploration} & \textbf{Scale-Up} \\ \hline
		\textbf{WordCount}      & 2.7\%            & 5.8\%    \\ 
		\textbf{Sort}           & 3.3\%            & 1.6\%    \\
		\textbf{TeraSort}       & 40.4\%           & 16.7\%   \\
		\textbf{RandomForest}   & 6.4\%            & 7.2\%    \\
		\textbf{SVD}            & 0.4\%            & 1.9\%    \\ \hline
% 		\textbf{LogisticRegression} & 17.5\%       & 27.4\%   \\ \hline
		\textbf{\textit{Average}} & 10.64\%       & 6.7\% \\
		\hline
	\end{tabular}
% 		~\chong{why did you put * in front of average?} Actually no reason, just a visual effect to distinguish Average with regular jobs.
\vspace{-.5cm}
\end{table}

==> tex/RQ1_b_2.tex <==
\begin{table}[t!]
    \caption{CPU time (secs) of default configuration for each job under three data inputs for Hadoop.}
    \label{tab:evaluation-time}	
    \arrayrulecolor{black}
    \setlength{\tabcolsep}{0.4cm}
    \centering
    \resizebox{\linewidth}{!}{
        \begin{tabular}{@{}lcccc}%P{1.5cm}}
            \toprule
            & \textbf{Small} & \textbf{Large} & \textbf{Huge} & \textbf{\#EXP}\bigstrut\\ \toprule
            \textbf{WordCount}  & 166.2          & 862.6          & 9367.1        & \#3241 (Gen17)\\
            \textbf{Sort}       & 133.4          & 869.8          & 9891.7        & \#3318 (Gen17)\\
            \textbf{Terasort}   & 115.7          & 1056.6         & 8751.6        & \#2876 (Gen15)\\
            \textbf{Pagerank}   & 300.0          & 5657.2         & 13096.1       & \#3177 (Gen16)\\
            \textbf{NutchIndex} & 477.9          & 6596.5         & 11215.7       & \#4685 (Gen24)\\ 
            \toprule
        \end{tabular}}%\\[-0.8em]%
        % 	~\chong{do you have similar data for Spark?} A: I don't have this data. The performance of Spark is wall-clock time, not CPU time.        
\end{table}
